Analyzing and Mitigating Data Stalls in DNN Training

Training Deep Neural Networks (DNNs) is resource-intensive and time-consuming. While prior research has explored many different ways of reducing DNN training time, the impact of input data pipeline, i.e., fetching raw data items from storage and performing data pre-processing in memory, has been relatively unexplored. This paper makes the following contributions: (1) We present the first comprehensive analysis of how the input data pipeline affects the training time of widely-used computer vision and audio Deep Neural Networks (DNNs), that typically involve complex data preprocessing. We analyze nine different models across three tasks and four datasets while varying factors such as the amount of memory, number of CPU threads, storage device, GPU generation etc on servers that are a part of a large production cluster at Microsoft. We find that in many cases, DNN training time is dominated by data stall time: time spent waiting for data to be fetched and preprocessed. (2) We build a tool, DS-Analyzer to precisely measure data stalls using a differential technique, and perform predictive what-if analysis on data stalls. (3) Finally, based on the insights from our analysis, we design and implement three simple but effective techniques in a data-loading library, CoorDL, to mitigate data stalls. Our experiments on a range of DNN tasks, models, datasets, and hardware configs show that when PyTorch uses CoorDL instead of the state-of-the-art DALI data loading library, DNN training time is reduced significantly (by as much as 5x on a single server).

==> abstract.tex <==
\begin{abstract}
  Training Deep Neural Networks (DNNs) is resource-intensive and
  time-consuming. While prior research has explored many different 
  ways of reducing DNN training time spanning different layers of the system stack,
  %by efficiently parallelizing training, or optimizing the GPU operators,
  the impact of \emph{input data pipeline}, i.e., fetching raw data items from storage and
  performing data pre-processing in memory, has been relatively unexplored.  
  
  This paper makes the following contributions: (1) We present the
  first comprehensive analysis of how the input data pipeline affects
  the training time of widely-used Deep Neural Networks (DNNs). We
  analyze nine different models across three tasks and four datasets
  while varying factors such as the amount of memory, number of CPU
  threads, storage device, GPU generation etc on servers that are a
  part of a large production cluster at Microsoft. We find that in
  many cases, DNN training time is dominated by \emph{data stall
    time}: time spent waiting for data to be fetched and
  pre-processed. (2) We build a tool, \tool to precisely measure data
  stalls using a differential technique, and perform predictive
  what-if analysis on data stalls.  (3) Finally, based on the insights
  from our analysis, we design and implement three simple but
  effective techniques in a data-loading library, \sysname, to
  mitigate data stalls.  Our experiments on a range of DNN tasks,
  models, datasets, and hardware configurations show that when PyTorch
  uses \sysname instead of the state-of-the-art DALI data loading
  library, DNN training time is reduced significantly (by as much as
  5\myx on a single server). 
  
  %Our analysis further motivates future research directions such as 
  %resource-aware data transformations, and a data layer abstraction
  %for DNN computation.


\end{abstract}

==> analysis.tex <==
\section{Analyzing Data Stalls}
\label{sec-analysis}

To understand data stalls in DNN training and 
the fundamental reasons why data stalls exist, 
we perform a comprehensive analysis
on several DNNs by varying a number of factors,
such as the number of GPUs, GPU generation, the size of the DRAM
cache, the number of CPU threads etc. We present our major
findings in this section, and show more analysis such as
impact of batch size and higher CPU cores in Appendix.

\subsection{Methodology}
\label{sec-methodology}
\vheading{Models and Datasets}. We analyze \textbf{nine}
state-of-the-art DNN models across three different tasks and four
different datasets as shown in Table~\ref{tbl-dataset-models}.  This
section focuses on the smaller ImageNet-1K dataset for image
classification models. Evaluation with large datasets like
ImageNet-22k and OpenImages is presented in
Section~\sref{sec-eval}. The image and audio classification models are
taken from TorchVision~\cite{torchvision} and
TorchAudio~\cite{torchaudio} respectively; for object detection, we
use NVIDIA's official release of SSD300
v1.1~\cite{nvidia-ssd}. For all DNNs, we use the same
pre-processing as in the original papers. Additionally, we evaluated data stalls on two
language models; Bert-Large pretraining~\cite{devlin2018bert} on Wikipedia \&
BookCorpus dataset~\cite{zhu2015aligning} for language modeling and
GNMT~\cite{wu2016google} on WMT16~\cite{wmt16} (EN-De) dataset for
translation. These models are GPU compute heavy and do not exhibit
data stalls in our training environment (hence, results excluded from analysis); 
data stalls may show up in these models if
GPUs get faster or the computation requirements for these models gets
lower due to compact model representations.


\input{tables/tbl-dataset-models}



\vheading{Training environment}. All experiments are performed on
PyTorch 1.1.0 using the state-of-the-art NVIDIA data loading pipeline,
DALI. We have empirically verified that DALI's performance is strictly
better than PyTorch, TF and MxNet's default data loaders; therefore we perform our analysis of data stalls using the strongest baseline, DALI.
We use two
distinct server configurations for our analysis as shown in
Table~\ref{tbl-analysis-sku}. Both these are part of a large production and research cluster
at Microsoft~\cite{philly,jeon2019analysis}, whose workload have guided the design
of several research systems for ML training~\cite{gandiva, tiresias, themis, gandiva-fair}.
These servers also closely resemble publicly available
cloud GPU SKUs~\cite{aws-p3, aws-p2}.
\confssd has configuration closest to
AWS p3.16xlarge~\cite{aws-p3} with gp2 storage~\cite{ebs}, while
\confhdd is closest to AWS p2.8xlarge~\cite{aws-p2} with st1
storage~\cite{ebs}.  Both our servers have 500GB DRAM, 24 physical CPU cores
, and 8 GPUs per server. 

\input{tables/tbl-analysis-sku}

\vheading{Training parameters}. For experiments on \confssd, we use a
batch size of 512 per GPU for all image classification models, 128 per
GPU for SSD-Res18, 16 per GPU for M5 and perform weak scaling
for distributed training (while ensuring that the global batch size is
consistent with those widely used in the ML community). Since V100
GPUs have tensor cores, we use Apex mixed precision training with LARC
(Layer-wise Adaptive Rate Clipping), and state-of-the art learning
rate warmup schedules~\cite{goyal2017accurate}. On \confhdd, we use
the maximum batch size that fits the GPU memory (less than 256 for all
models) and perform full-precision training.

\vheading{Training metrics}. We run all the experiments presented here
for three epochs, and report the average epoch
time (or throughput in samples per second), ignoring the first epoch.
Since we start with a cold cache in our experiments, first epoch is
used for warmup. Measuring data stall
time does not require training to accuracy; per-epoch time
remains stable.




\subsection{Measuring data stalls using \tool}
\label{sec-tool}
We develop a standalone tool, \textit{\tool} that profiles data stalls
in DNN training.  Frameworks like PyTorch and TensorFlow provide an
approximate time spent on data loading and pre-processing per
minibatch, by simply placing timers in the training script. This is
insufficient and inaccurate for two reasons.  First, this technique
cannot accurately provide the split up of time spent in data fetch (from disk or
cache) and pre-processing operations. To understand if the training is
bottlnecked on \vio or CPU, it is important to know this split. Second,
frameworks like PyTorch and libraries like DALI use several concurrent
processes (or threads) to fetch and pre-process data; for
a multi-GPU data parallel training job, a data stall in one of the
data loading processes may reflect as GPU compute time for the other
processes, because all GPU processes wait to synchronize weight
updates at batch boundaries. Naively adding timers around data path
does not provide accurate timing information. Therefore, \tool uses a
differential approach.  \tool runs in three phases;
\begin{enumerate}[noitemsep,topsep=0pt,parsep=0pt,partopsep=0pt,leftmargin=18pt]
	
\item \vheading{Measure ingestion rate}.
  First, \tool pre-populates synthetic data at the GPUs and runs the job for a
  fixed number of epochs.
      This identifies the max data ingestion rate at the GPUs,
      with no fetch or prep stalls.
	\item \vheading{Measure prep stalls}. Next, \tool
	runs the training script with a subset of the given dataset,
	such that it is entirely cached in 
	memory, using all available CPU cores, and estimates the training speed. Since this run 
	eliminates fetch stalls, any drop in throughput compared
	to (1) is due to prep stalls.
	\item \vheading{Measure fetch stalls}. Finally,
	\tool runs the training script by clearing all caches, 
	and setting maximum cache size to a user-given limit, to
	account for fetch stalls. The difference between (2)
	and (3) is the impact of fetch stalls.
\end{enumerate}



%Additionally, \tool collects
%low level metrics such as the throughput of the storage device,
%memory and network bandwidth, cache size, and memory
%utilization.


\subsection{Data Stalls in DNN Training}
\label{sec-data-stall}
Our analysis aims to answer the following
%important
questions:
\input{tables/tbl-analysisq}

\begin{comment}
%with respect to data stalls in DNN training.
\begincompactitemize
      \item \vheading{Fetch Stalls (Remote)}. When does the remote storage
(distributed filesystem/object stores) become a bottleneck for DNN training? (\sref{sec-fetch-remote})
	\item \vheading{Fetch Stalls (Local)}. When does the local storage device
      (SSD/HDD)
      become a bottleneck for DNN training? (\sref{sec-fetch})
	\item \vheading{Prep Stalls}. When does data augmentation at the CPU 
	become a bottleneck for DNN training? (\sref{sec-prep})
	\item \vheading{Generality}. Do fetch and prep stalls exist in other training platforms like TensorFlow? (\sref{sec-tf})
\end{itemize}
\end{comment}
\subsubsection{When dataset resides on remote storage}
\label{sec-fetch-remote}
Datasets used for training DNNs could reside locally on the persistent storage of a 
server, or on shared remote storage such as distributed file systems (HDFS, GlusterFS - GFS),
or object stores (S3, Azure blobs). We analyze the impact of two kinds of remote backends;
a distributed file system, GlusterFS (GFS) and the Azure blob object store accessed via blobfuse. 

When data resides remotely, the first epoch of training fetches data
over the network and stores it locally for subsequent use. Cluster
file systems like GFS use the OS Page Cache to speed up subsequent
accesses. Blobfuse downloads the dataset on to local SSD, and mimics
local training from the second epoch.  Figure ~\ref{fig-remote}a
compares the epoch time for ResNet18 on \confssd using GFS, blobfuse,
and local SSD for the first epoch and a stable-state epoch with warmed
up cache.


The data stall overhead of BlobFuse is especially high in the first
epoch when it downloads the entire dataset to local storage, and can
result in 20\myx higher training time as compared to GFS. 
Unsurprisingly, during the steady state epochs, data stall
overheads when using the local SSD and BlobFuse are similar (as the
blob data is cached on the local SSD); GFS results in more data stalls
as it validates metadata of cached data items over the network every
time a data item is accessed. Blobfuse does not incur any network
cost beyond first epoch, if the dataset fits on local SSD.

As shown in Figure~\ref{fig-remote}b, for the ImageNet1K dataset,
for BlobFuse, the cost of downloading the entire dataset in the first
epoch is amortized as we train for a longer number of epochs, making
the remote Blobstore a better fit compared to GFS when models are trained to accuracy
for over 60 epochs.

Athough datasets are growing in size, large datasets that are
publicly available fit entirely on local storage (but not in memory)~\cite{training-big,
	abu2016youtube, kuznetsova2018open, defferrard2016fma, imagenet-22k, russakovsky2015imagenet}.
Therefore, a common training scenario is to pay a one-time download
cost for the dataset, and reap benefits of local-SSD accesses
thereafter (default and recommended mode in the Microsoft
clusters). Therefore, in the rest of the work, we analyze fetch stalls
in scenarios where dataset is present locally on a server, but is not
entirely cached in memory.

\input{fig-analysis/fig-remote}

\subsubsection{When datasets cannot be fully cached}
\label{sec-fetch}
%Datasets used for training DNNs are growing in
%size~\cite{training-big, abu2016youtube, kuznetsova2018open}. Even the
ML-optimized cloud servers with 500GB DRAM can only cache 35\%
of ImageNet-22K, or 45\% of the FMA dataset, or 65\% of the OpenImages
dataset, although they entirely fit on local storage. 
Popular datasets like ImageNet-1K cannot be fully cached on
commonly used cloud SKUs like AWS \vtt{p3.2xlarge}, which has 61 \gb
DRAM. When datasets don't fit in memory, and the fetch rate($F$)
%is less
%than the
$<$
compute rate ($min(P,G)$), fetch stalls occur.
%Such scenarios 
%may result in \textbf{fetch stalls}
%during training, which might result in the training job
%being I/O bound due to constant disk activity. 
%The experiments in this section limit the
%memory available to the docker container to simulate different
% caching scenarios and analyze storage bottleneck.


\begin{comment}
\vspace{0.5em}
\begin{mybox}
	\textit{\textbf{1. Fetch stalls are common if dataset is not fully cached in memory}}
\end{mybox}
\vspace{-0.5em}
\end{comment}

\vheading{Fetch stalls are common if the dataset is not fully cached in memory}.
Figure~\ref{fig-analysis-cache-dnn} shows the percentage of per 
epoch time spent on \vio for nine different DNNs when 35\% ( for \eg ImageNet-22k on 500GB server) 
of their respective
datasets can be cached in memory on \confssd. DNNs spend 10 --70\% of their epoch
time on blocking \vio, despite pipelining and prefetching, simply
because the compute rate is higher than fetch rate.


\begin{comment}
\vspace{0.5em}
\begin{mybox}
\textit{\textbf{2. OS Page Cache replacement policies are inefficient for single-server training jobs}}
\end{mybox}
\vspace{-0.5em}
\end{comment}



\vheading{OS Page Cache is inefficient for DNN
  training}. DNN training platforms like PyTorch, TensorFlow and
libraries like DALI, rely on the operating system's Page Cache to
cache raw training data in memory. Unfortunately, the OS Page Cache
leads to thrashing as it is not efficient for DNN training. \emph{If 35\% of
the data can be cached, then an effective cache should provide 35\%
hits; instead, the Page Cache provides a lower hit rate}. For a 146
\gb data set, each epoch should see only 65\% of the dataset, or 95\gb,
fetched from storage. Instead, we observe 85\% of the dataset fetched
from storage every epoch; the 20\% difference is due to
thrashing. Figure~\ref{fig-analysis-cache-res18} shows the fetch
stalls, including those due to thrashing, when using PyTorch with
DALI. An effective cache for DNN training must eliminate thrashing to
reduce fetch stalls to the minimum shown in
Figure~\ref{fig-analysis-cache-res18}.


\begin{comment}
\vspace{0.5em}
\begin{mybox}
	\textit{\textbf{3. Uncoordinated local caches make multi-server single-job training IO bound}}
\end{mybox}
\vspace{-0.5em}
\end{comment}



%\vheading{Takeaway 3 : Uncoordinated local caches make multi-server
%  training IO bound}.
\vheading{Lack of coordination among caches leads to
  redundant \vio in distributed training}. In distributed training
jobs, the data to be fetched and processed is divided randomly among
servers, and changes every epoch. As a result,
each server often has to fetch data from storage every epoch; this is
done even if the required data item is cached in an another server that is a part
of the distributed training job. This lack of coordination among
caches makes distributed training storage \vio-bound. 
When training Resnet50 on ImageNet-1K (146\gb) across
two servers having a total cache size of 150\gb, each server fetches
45\gb from storage in each epoch (despite the fact that the 
other server might have this data item in its cache). 
On \confhdd, this leaves ResNet50 stalled on \vio for 75\% of its epoch time.

\input{fig-analysis/fig-analysis-cache-dnn}
\input{fig-analysis/fig-analysis-cache-res18-both}


\begin{comment}
\vspace{0.5em}
\begin{mybox}
	\textit{\textbf{4. Uncoordinated data access pattern of HP search jobs result in large read amplification}}
\end{mybox}
\vspace{-0.5em}
\end{comment}

%\vheading{Takeaway 4 : Uncoordinated data access pattern of HP search
%  jobs result in large read amplification}.
%\input{tables/tbl-analysis-cache-hp}
\vheading{Lack of coordination in HP search results in
  redundant \vio}. HP search is performed by launching several
parallel jobs with different HP on all available GPUs in
a server~\cite{liaw2018tune}. All HP jobs access the same dataset in a
random order in each epoch, resulting in cache thrashing and read
amplification.
When 8 single-GPU jobs are run in a server (35\% cache), there is 7\myx read amplification per
epoch (884 \gb read off storage compared to 125 \gb for one job), 
which slows down HP search on ResNet18 by 2\myx on \confssd.

\input{fig-analysis/fig-prep}
%\input{fig-analysis/fig-analysis-prep-cpu}
\input{fig-analysis/fig-analysis-prep-res18}
%\input{fig-analysis/fig-analysis-prep-all}
\input{fig-dali/fig-frameworks}

\subsubsection{When datasets fit in memory}
\label{sec-prep}


We now analyze the impact of CPU pre-processing on DNN training in the
scenario where the entire dataset is cached in memory of a single server, thus
eliminating fetch stalls due to storage \vio.

\begin{comment}
\vspace{0.5em}
\begin{mybox}
	\textit{\textbf{5. DNNs need 3 -- 24 CPU cores per GPU for pre-processing}}
\end{mybox}
\vspace{-0.5em}
\end{comment}

\vheading{DNNs need 3--24 CPU cores per GPU for
  pre-processing}.  Figure~\ref{fig-analysis-prep-cpu} shows how DNN
training throughput changes as we vary the number of CPU
pre-processing threads (per V100 GPU) for four models. For computationally
complex models like ResNet50, 3 -- 4 CPU cores per
GPU is enough to prevent prep stalls; for computationally lighter models
like ResNet18 or AlexNet, as many as 12 -- 24 CPUs per GPU are needed
to mask prep stalls. %Since prep is CPU-intensive, using 
%more threads (vCPUs) than the number of physical CPU cores does not help
%much; For a 8-GPU server with 32 CPU cores (64vCPUs), ResNet18 
%spends 37\% of the epoch time on prep stalls (Appendix).
Even on NVIDIA's AI-optimized DGX-2,
there are only three CPU cores per GPU; thus, many models have prep
stalls on the DGX-2 (~\sref{sec-dgx2})



\begin{comment}
\vspace{0.5em}
\begin{mybox}
	\textit{\textbf{6. Prep stalls exist across various GPU configurations, even with GPU based prep}}
\end{mybox}
\vspace{-0.5em}
\end{comment}

%\vheading{Takeaway 6 : Prep stalls exist across various GPU configurations, even with DALI}. 

\vheading{DALI is able to reduce, but not eliminate prep
  stalls}. DALI uses the GPU for pre-processing operations, and is
thus able to reduce prep stalls, as shown in
Figure~\ref{fig-analysis-prep-res18} (a). The effectiveness of DALI
depends on the GPU speed; for example, on the slower 1080Ti, DALI is
able to eliminate prep stalls using three CPU threads per GPU. On
the faster V100 though, DALI still results in 50\% prep stalls when
using three CPU threads per
GPU. Figure~\ref{fig-analysis-prep-all} shows that our observations
hold across different DNNs when training with eight GPUs each with 3 CPUs.

\vheading{Decoding is very expensive!}
To understand what makes prep expensive, we
run a microbenchmark to breakdown the cost of different stages
in a typical prep pipeline for image classification tasks.
An input image is first loaded into memory, decoded, and then randomly
transformed (crop, flip), and finally copied over to the GPU as a tensor that
can be processed. Fig ~\ref{fig-prep-breakdown} shows the time 
taken for each operation when prep is done on CPU and GPU by DALI. 
%In the GPU-based
%$prep, decode operation is partly done on CPU and then offloaded to GPU. All subsequent operations
%are performed at the GPU. There are two main takeaways from this graph. 
%First, 
We see that offloading 
prep to the GPU provides significant speedup at the expense of GPU memory usage (+5GB!). 
%5.5GB of GPU memory is consumed in this case, which adversely affects the maximum batch size 
%that a model can use for training. Furthermore, for models that are already GPU-intensive, 
%offloading the prep pipeline interferes with training and results in reduced throughput
%(ResNet50, VGG). 
Second, a majority of time during prep is spent in decoding images. 


% I think tabkle is unnecessary. Can explain the insight 
% using all results so far
%\input{tables/tbl-analysis-prep-hp}
\begin{comment}
\vspace{0.5em}
\begin{mybox}
    	%\sepline
		\textit{\textbf{7. Redundant pre-processing in HP search results in high prep stalls}}
\end{mybox}
\vspace{-0.5em}
\end{comment}



\vheading{Redundant pre-processing in HP search results
  in high prep stalls}.  During HP search, concurrent jobs process the
same data. Currently, there is no coordination; if there are 8 HP
jobs, the same data item is processed eight times. This is made worse
by the fact that all HP jobs share the same set of CPU threads,
leading to fewer CPU threads per GPU, and higher prep
stalls. When 8 single-GPU ResNet18 HP jobs run on \confssd, each job gets 3 CPU
for prep and incurs a 50\% prep stall as shown in  
Figure~\ref{fig-analysis-prep-all}. Coordinating these HP search jobs on a single 
server can potentially eliminate prep stalls, as all available CPU
(24 cores) can be used to prep the dataset exactly once per epoch and reused across jobs
(Figure~\ref{fig-analysis-prep-cpu} shows ResNet18 requires 12 CPUs per GPU to
eliminate prep stalls).

%\input{tables/tbl-tensorflow-small}


\subsubsection{Data stalls exist across training frameworks}% and data formats}
\label{sec-tf}

\begin{comment}
\vspace{0.5em}
\begin{mybox}
	\textit{\textbf{8. Data stalls exist across training frameworks} % and data formats}}
\end{mybox}
\vspace{-0.5em}
\end{comment}

%\input{tables/tbl-analysis-summary}

%\vheading{Takeaway 8 : Data stalls exist across training frameworks and data formats}
To generalize our findings on data stalls across different training
platforms and data formats, we analyze the prep and fetch stalls in
TensorFlow (TF) using the binary TFRecord format, and MxNet using RecordIO format. 
Unlike
PyTorch, TF does not store training data as small individual
raw files. Instead, it shuffles the small random files, serializes
it, and stores them as a set of files (100-200MB each) called
TFRecords. TFRecords make reads more sequential. MXNet also use a similar serializing technique for data called
RecordIO~\cite{recordio}.
%We evaluate TensorFlow as a representative
%candidate for such record formats.


Figure~\ref{fig-analysis-framework-prep} shows that both native
TF and MxNet spend 65\% and 50\% of the epoch time on prep stall
for a 8-GPU ResNet18 training job when the dataset is entirely
cached in memory.
Next, Table~\ref{tbl-analysis-tf-small} shows the percentage of misses in
the Page Cache for a 8-GPU training job and the \vio amplification due
to lack of coordination in HP search for varying cache sizes in TF. %Similar to PyTorch, TF
%can also use DALI's GPU based pre-processing and exhibit prep stalls
%similar to PyTorch.  
TFRecord format results in 40\%
higher cache misses than the ideal because, the sequential access
nature of TFRecords (and RecordIO) is at odds with LRU cache replacement policy of
the Page Cache, resulting in a pathological case for LRU
(this is 20\%higher than PyTorch).  
The lack of co-ordination
in HP jobs results in upto 7.2\myx read amplification; although
all jobs read the same 140 \gb dataset, the total disk \vio was 1.1
TB.


\subsubsection{Analysis summary}
Table~\ref{tbl-summary} summarizes our key 
findings pertaining to data stalls across DNN training frameworks, models, and
hardware configurations.
Our analysis shows that mitigating data stalls is of paramount importance
to exploit the performance benefits of fast accelerators. Furthermore, it throws
light on the need for specialized, domain-specific techniques such as 
bypassing the OS Page Cache, and coordinating individual jobs, to eliminate data stalls.

%also highlights that data stalls are a consistent problem across both TensorFlow and PyTorch.


==> disc.tex <==
\subsection{Limitations and Future Work}
\label{sec-disc}

Our analysis of data stalls reveals several key insights to
utilize the computational capabilities of GPUs by minimizing
data stalls. While we explore ways of mitigating
data stalls in a user-space library \sysname, we believe there is
more to be done. 

\sysname does not address the high cost of image decoding 
which our analysis identifies to be the most expensive
operation during data prep. A future direction is to evaluate the 
benefits of caching decoded 
data items instead of the current approach of caching raw encoded items. 
Since decoding is deterministic, it is possible to
cache it across epochs. However, this is non trivial; 
decoding blows up the size of data item by  5 -- 7 \myx.
It is an interesting future direction to enable decoded caching
without incurring the high space overhead, possibly using serialized
data formats.


==> existing.tex <==
Before we design and evaluate new techniques, we first investigate the
approaches used by recent works like 
Quiver~\cite{kumar2020quiver}, DeepIO~\cite{zhu2018entropy},
and Cerebro~\cite{cerebro} that build systems for large-scale distributed training. 
These works have identified that data fetch from remote
storage can bottleneck large-scale distributed DNN training. 
We now discuss how each one
of these systems fall short of harnessing the insights from our analysis, and
the need for a coordinated caching and pre-processing library for DNN training.

\subsection{Limitations of Existing Work}
\vheading{When even data is cached on local storage, there are data
  stalls}.  Prior work targets distributed training scenarios, and use
techniques like data partitioning across servers to mitigate the low
throughput of remote storage.  The partitioned dataset is cached on
local SSD (Quiver~\cite{kumar2020quiver}), or local memory
(Cerebro~\cite{cerebro}, DeepIO~\cite{zhu2018entropy}).  However, our
analysis shows that even if data is cached locally in memory or on
SSDs, data stalls can still exist due to inefficient caching or
expensive pre-processing. An efficient data pipeline should therefore
help even when the data is locally cached. 

\vheading{Ignoring DNN ETL requirements}. Prior work like Cerebro and
OneAccess~\cite{kakaraparthy2019case} make a compelling case for
caching pre-processed data items and reusing it across epochs.  While
this would mitigate prep stalls, it defies the DNN ETL requirements
(~\sref{sec-etl}). Not shuffling data items across partitions every
epoch, and reusing the same pre-processed items across epochs have
been shown theoretically and empirically to affect the convergence of
SGD for DNN training~\cite{convergence}. Therefore, we need a data
pipeline that efficiently \emph{supports all ETL requirements}, while
mitigating prep stalls.

\vheading{Intrusive infrastructure changes}. Deploying techniques used
in prior work needs infrastructure-level changes such as deploying a
cache manager (Quiver), scheduler (Cerebro), or specialized hardware
like RDMA (DeepIO) in the cluster. This requires significant effort
%to be deployed and used in practice 
in large production clusters. A practical, user-friendly solution
should require \emph{no intrusive cluster infrastructure changes}, and
be capable of harnessing the hardware resources allocated to the job
efficiently.

\vheading{Our solutions}.  The insights from our analysis must be
incorporated in (1) a user-space library that can be used by
individual training jobs (2) with no cluster infrastructure changes,
and (3) mitigate data stalls while supporting all the DNN ETL
requirements. We now discuss three techniques to mitigate data
stalls.% as shown below. %in Table~\ref{tbl-techniques}.


==> fig-analysis/fig-analysis-cache-res18.tex <==
\begin{figure}[!t]
  \centering 
   \includegraphics[width=.49\textwidth, height=4cm]{graphs-dali/analysis-cache-1.png}
   \vspace{-2em}
  \mycaption{ResNet18 with varying cache}{A closer look at the disk activity reveals that,
  even with a single training job, the cache is used inefficiently due to thrashing.}
  \vspace{-3em}
  \label{fig-analysis-cache-res18}
\end{figure}

==> fig-analysis/fig-analysis-prep-all.tex <==
\begin{figure}[!t]
  \centering 
   \includegraphics[width=.45\textwidth]{graphs-dali/analysis-prep-all.png}
    \vspace{-1em}
  \mycaption{Prep stall across DNNs}{This graph plots prep stall as a percentage of the epoch time, when training various DNNs across 8-GPUs on \confssd. DNNs spend 5 -- 65\% of their epoch time on blocking prep.}

  \label{fig-analysis-prep-all}
\vspace{-0.8em}
\end{figure}

==> fig-analysis/fig-analysis-prep-cpu.tex <==
\begin{figure}[!t]
  \centering 
   \includegraphics[width=.43\textwidth]{graphs-dali/analysis-prep-cpu-speed.png}
  
  \mycaption{Impact of CPU cores on training}
  	% of different image classification models}
  	{DNNs need between 3 -- 24 cores per GPU
  to mask prep stalls.}
  \vspace{-1em}
  \label{fig-analysis-prep-cpu}

\end{figure}

==> fig-analysis/fig-prep-breakdown.tex <==
 \begin{figure}[!t]

  \centering 

  \includegraphics[width=.4\textwidth]{graphs-dali/prep_breakdown.png} 
   
  
    \mycaption{Breakdown of prep overhead}{This graph shows the split up of
    time spent on each phase of prep for a image classification workload on 
ImageNet-1k. GPU-based prep is significantly faster than CPU-based, at the expense 
of additional GPU memory usage. Decoding images takes the most time in the pipeline.}

  \label{fig-prep-breakdown}

\end{figure}

==> fig-analysis/fig-tool-combined.tex <==
\setlength\mylength{\dimexpr.5\columnwidth-10\tabcolsep-0.5\arrayrulewidth\relax}

\begin{figure}[!t]
	\centering
	\begin{tabular}{l}
		\kern-0.5em\subfloat[100\% Cache \label{fig-analysis-framework-prep}]{\adjustbox{raise=-2.6pc}{\includegraphics[width=5cm]{graphs-dali/tool.png}} }
		\quad
		\kern-0.5em\subfloat[TensorFlow (Vary cache)
		\label{tbl-analysis-tf-small}]{
		 \begin{tabular}{@{}c|c|cc@{}}
			\toprule[1.2pt]
			%      & \multicolumn{3}{c}{\% dataset cached}\\
			\% cached  &   8-GPU job & \multicolumn{2}{c}{8-job HP}\\
			(Sz:146GB) &  Cache Miss	   &   IO(GB) & Read amp \\
			\midrule
			50\% & 91\% & 860 &  6.14\myx \\
			35\% & 94\% & 1010 & 7.21\myx \\
			25\% & 97\% &  1019 & 7.28\myx \\
			\bottomrule[1.2pt]
		\end{tabular}
		}%
		\label{fig-analysis-frameworks}
	\end{tabular}
\vspace{-1em}
	\mycaption{Data stalls across frameworks}{The plot shows that data stalls exist in other training frameworks like MxNet and TensorFlow in various training scenarios.}
	\vspace{-1em}
\end{figure}

==> fig-dali/fig-accuracy.tex <==
\begin{figure}[!t]

  {\includegraphics[width=0.85\columnwidth]{graphs-dali/accuracy.png}}
     \vspace{-8pt}
  \mycaption{Top-1 validation accuracy during training}{In training ResNet50 with ImageNet-1K on 16x 1080Tis across 2 servers, \sysname reduces the time to accuracy by 4\myx by coordinating the caches across the job's individual servers.}
  \label{fig-accuracy}
  \vspace{-5pt}
\end{figure}


==> fig-dali/fig-dgx2.tex <==
 \begin{figure}[!t]

  \centering 

  \includegraphics[width=.4\textwidth]{graphs-dali/dgx-coordl.png} 
   
  
    \mycaption{Evaluation of \sysname on DGX-2}{This graph compares DALI against
      \sysname for HP search using 16 GPUs on the state-of-the-art ML optimized 
  	server DGX-2. \sysname outperforms the best GPU-based prep mode of DALI which uses 5GB of GPU memory 
  for pre-processing. \sysname allows training larger batch sizes, while providing better performance than 
DALI.}

  \label{fig-dgx2}

\end{figure}

==> fig-dali/fig-hp-split.tex <==
 \begin{figure}[!t]

  \centering 

  \includegraphics[width=.4\textwidth]{graphs-dali/eval-split.png} 
   
  
    \mycaption{Comparison of \sysname to fetch-only coordination techniques}{This graph compares DALI and \sysname against
     coordinated fetch techniques used by Quiver for HP search. HP search jobs are primarily stalled on data prep; eliminating redundancy in fetch alone (used by Quiver) does not mitigate data stalls completely.}

  \label{fig-eval-split}

\end{figure}

==> fig-dali/fig-mint-io.tex <==
\begin{figure}[!t]

  {\includegraphics[width=0.85\columnwidth]{graphs-dali/mint-io.png}}
   \vspace{-7pt}
  \mycaption{Disk I/O pattern with \minio (ResNet18 on OpenImages)}{DALI gets cache hits at the start of every
    epoch; however due to thrashing, all requests result in storage
    access beyond a point. \sysname results in a more uniform \vio
    pattern and faster training.
  }
  \label{fig-mint-io}
  \vspace{-4mm}
\end{figure}


==> fig-dali/fig-processing-rate-res18.tex <==
\begin{figure}[!t]
  \centering
  %\includegraphics[width=0.47\textwidth]{graphs-dali/processing-rate-res18.pdf}
  \includegraphics[width=0.95\columnwidth]{graphs-dali/pipeline-abstract.pdf}
  %\vspace{-16pt}
  \mycaption{Data Pipeline for ResNet18}{This figure shows the data
    pipeline with DALI for the ResNet18 model along with the
    throughput of each component in the pipeline.  On a server with 8
    \vtt{V100} GPUs and 24 physical CPU cores, the overall throughput of the data
    pipeline is lower than the expected ingestion rate at the GPU,
    resulting in data stalls.} 
    \vspace{-3mm}
  \label{fig-processing-rate-res18}
\end{figure}


==> fig-dali/fig-recall.tex <==
\begin{figure}[!t]

  {\includegraphics[width=0.8\columnwidth]{graphs-dali/coordl.pdf}}
   \vspace{-0.7em}
  \mycaption{Architecture of \sysname}{%Raw data items from the local
    %storage are cached in the \minio cache. Multiple CPU
    %threads fetch items from the local (or remote) \minio cache, pre-process and create
    %minibatches, which are then staged for sharing across jobs,
    %if there are multiple jobs.
}
  \label{fig-recall}
  \vspace{-2.5em}
\end{figure}


==> intro0.tex <==
\section{Introduction}
\label{sec-intro}

% Lets hope the 5th time is the charm.
% Intro v5

% ML and DNN together
Machine learning has become pervasive in our lives. It is used both in
user-facing applications and in the backend infrastructure. One class
of machine-learning models, Deep Neural Networks (DNN), have gained
importance as they allow us to tackle problems that were previously
intractable, such as image
classification~\cite{krizhevsky2012imagenet,simonyan2014very,he2016deep},
translation~\cite{wu2016google}, speech
recognition\cite{graves2013speech}, video
captioning~\cite{venugopalan2015sequence}, and even predictive
health-care~\cite{deepmind-health}.

Training DNNs is resource-intensive and time-consuming. During
training, the model predicts the output given training data; based on
the output, the model's weights are tuned. This happens iteratively,
in many rounds called epochs. The training process uses configuration
options called hyperparameters (HP) that influence the speed and
quality of the learning process. So the first step in training a model
is finding the optimal set of HP. HP search is typically performed by
launching several parallel jobs with different hyperparameters,
monitoring their progress, and replacing poorly performing ones with
new values, until the best hyperparameters are found.  Once the
hyperparameters are decided, DNN training is performed on a single
GPU, single server with multiple GPUs, or across multiple servers in a
cluster.

Training a DNN, especially in the distributed setting, involves all
the different resources in a server from GPUs to networking. 
%Training a DNN involves the holistic use of datacenter hardware: storage systems to
%read datasets, CPUs to preprocess input data, hardware accelerators to
%perform DNN computations, and communication networks to facilitate
%distributed training.
Researchers have tackled how to efficiently use these
resources to reduce DNN training time,
%Researchers have tackled reducing DNN training time using a number of
%different approaches
such as reducing communication
overhead~\cite{lin2017dgc, PoseidonATC2017, hashemi2018tictac,
  jayarajan2019priority, narayanan2019pipedream}, GPU memory
optimizations~\cite{vdnn,chen2016training, gist2018}, and
compiler-based operator optimizations~\cite{vasilache2018tensor,
  chen2018tvm,jia2019taso}.
%However, the impact of the \emph{data
% pipeline} on DNN training has been relatively unexplored.
However, the impact of storage systems, specifically the \emph{data
  pipeline}, on DNN training has been relatively unexplored.

During DNN training, the data pipeline works as follows.  Data items
are first fetched from storage and then \emph{pre-processed}. 
For example, for many important and widely-used
classes of DNNs that work on images, audio, or video, there are
several pre-processing steps: the data is first decompressed,
and then random perturbations such as cropping the image or rotating
it are performed to improve the model’s
accuracy~\cite{perez2017effectiveness}.
%Training proceeds in multiple
%rounds called epochs, and
Pre-processing with the required random transformations has to be done
for each epoch, while ensuring that each item in the dataset is
processed exactly once per epoch.  Once pre-processed, the data items
are sent to the GPUs for processing. This data fetch and
pre-processing is normally pipelined with the GPU computation.
Ideally, the data pipeline should keep the GPUs continuously busy
processing data; we term this GPU-bound. Unfortunately, DNN training
is often IO-bound, bottlenecked by fetching the data from storage, or
CPU-bound, bottlenecked by pre-processing data in
memory. Collectively, we term these bottlenecks \emph{data stalls} and
differentiate between \emph{prep stalls} (time spent pre-processing)
and \emph{fetch stalls} (time spent on IO).

% the contributions para
\vheading{Contributions}. We present the first comprehensive analysis
of data stalls across nine popular DNN models from three domains
(image classification, object detection, and audio classification) and
four datasets.  We vary factors such as the storage media (hard disks
and SSDs), amount of data that can be cached in memory, the number of
CPU threads used to fetch and pre-process data, the number of GPUs,
and GPU generation.  We then analyze how these factors affect the data
pipeline and DNN training. We find that the data pipelines in popular
training frameworks like PyTorch and TensorFlow are inefficient,
despite using state-of-the-art data-loading libraries like
DALI~\cite{noauthor_fast_2019} that reduce prep stalls using
GPU-accelerated data pre-processing. We present \sysname, a novel data
loading library that accelerates DNN training by minimizing data
stalls. \sysname does not impact accuracy; training can sample as
usual from the entire dataset, regardless of what is cached. \sysname
does not require specialized hardware, and runs over commodity
networking and storage hardware.  \sysname addresses both fetch and
prep stalls and accelerates several common training scenarios: HP
search (by upto 5.7\myx), single-server DNN training (by upto 2\myx),
and multi-server DNN training (by upto 15\myx).

Performing an analysis of how the data pipeline impacts DNN training
is challenging since DNN training has a high degree of concurrency; it
is hard to isolate the time taken to perform a single task especially
as data loading and preparation are pipelined with GPU computation.
We develop a tool, \tool, that uses differential analysis between runs
(\eg comparing a run where data is completely cached vs when data
needs to be fetched from storage) to accurately identify data-stall
bottlenecks.


Our analysis yields several interesting insights. 
First, a large number of DNN models, even computationally expensive ones like ResNet50~\cite{he2016deep} and
VGG11~\cite{simonyan2014very}, have data stalls.
Second, these data stalls occur across frameworks such as PyTorch and TensorFlow.
Third, some models like ResNet18 require more than three cores per GPU for
pre-processing; these models have prep stalls even on ML-optimized
hardware like DGX-2~\cite{dgx2}.
Fourth, there is a large amount of redundant work done by the
data pipeline during HP search and distributed
training where the same data items are fetched and pre-processed
 by multiple jobs or multiple servers. 
Finally, when the dataset is larger than available
memory, current caching policies used by DNN training frameworks are
inefficient, resulting in high disk I/O with unwanted evictions in the Page Cache. 

For example, consider a cluster of ML-optimized cloud servers with
V100 GPUs and 500 \gb of memory~\cite{aws-p3}; 400\gb is allocated to
cache the input dataset. We would like to train
ResNet50~\cite{he2016deep} using the 645 \gb
OpenImages~\cite{kuznetsova2018open, sarincrowdsource} dataset in
PyTorch with DALI.  When we perform HP Search for this model with
eight jobs on a single server, a staggering 1.7 \tb of data (2.8\myx
the size of the entire dataset) is fetched from storage during
\emph{each} epoch because the data pipeline of each of the eight jobs
fetches and pre-processes the dataset independently. After determining
the hyperparameters, when we perform distributed training on 16 GPUs
across two servers, in each epoch of training both servers process a
random disjoint half of the dataset (so that they collectively process
the entire dataset once per epoch). Despite enough memory across two
servers (800 \gb) to cache the entire dataset, each server fetches 119
\gb (from storage) per epoch when training, as the random data items
being requested may not be cached locally at each server.  If the
server uses hard drives for storage, training incurs fetch stalls,
%when there is not enough memory to cache the entire dataset, 
causing the expensive GPU to be idle for
75\% of the total training time.

\begin{comment}

There have been recent efforts such as Quiver~\cite{kumar2020quiver}, Pure Storage's AI Ready Infrastructure (AIRI)~\cite{}, and DeepIO~\cite{zhu2018entropy} that aim at speeding up data fetch times.
But such approaches have limited applicability as they either don't tackle prep stalls, don't work for distributed training, might impact accuracy because they violate the invariant that every data item is used once every epoch (by using only cached items), or use specialized storage and hardware like RDMA.
\jm{The description is inaccurate. Quiver does not break the
invariant. And maybe we can get rid of DeepIO from here and 
talk only in related work, }
\ap{feel free to fix it! :-)}


While recent work such as Quiver~\cite{kumar2020quiver} and
DeepIO~\cite{zhu2018entropy} aim at reducing data fetch time, 
they are designed for specialized training
scenarios such as multi-tenant clusters where
the dataset is too large to fit on local storage device (>3TB), or
large scale HPC systems with specialized hardware like RDMA 
(which are not available on commodity cloud GPU servers) respectively.
However, they do not address the more common, single user training scenarios over
commodity hardware.
%Furthermore, they might impact accuracy when they can
%cache only a portion of the data, as they restrict sampling to only cached items.
%\ap{I'd omit or rework the related work lines above, because of two reasons: 
%the immediately preceding line is unclear and it begs comparison to these systems in eval.}
%\jm{Does this help?}
\vc{rewrite to say what the fundamental issues are? If too long, might
  as well leave for related work section}
  
\end{comment}

Using the insights from our analysis as opportunities for improvement,
we design and build \sysname, a novel data loading library that
accelerates DNN training by minimizing data stalls. \sysname
introduces three techniques to overcome data stall overheads.
First, it introduces \emph{coordinated prep}, which coordinates data
fetch and pre-processing among concurrent HP search
jobs. Coordinated prep takes advantage of the fact that all HP jobs
are operating on the same data; all concurrent jobs can share one
epoch's worth of pre-processed data. In each epoch, data is fetched
and pre-processed exactly once for all concurrent HP jobs, eliminating
a significant amount of redundant work.
%Pre-processed data is not
%cached or used across epochs in a job to ensure model convergence.
Second, \sysname introduces the novel \minio software cache that is
specialized for DNN training. \minio exploits the unique data access
pattern in DNN training to minimize the amount of data fetched from
storage for training on a single server.
Third, \sysname introduces \emph{partitioned caching}, where the
dataset is partitioned and cached among the servers involved in distributed
training for each job.  On a local \minio cache miss, data is fetched from the memory of a
remote server (over the commodity TCP stack) rather than from local
storage. The dataset is thus fetched from storage exactly once for the
entire distributed training job.


%\sysname introduces \emph{partitioned caching}, where the dataset is
%partitioned and cached among the servers in distributed training. On a
%cache miss, data is fetched from the memory of a remote server (using a
%commodity TCP stack) rather than from local storage. The dataset is
%fetched from storage exactly once for the entire cluster. Finally,
%\sysname introduces the \minio software cache specialized for DNN
%training which eliminates thrashing and minimizes the amount of data
%fetched from storage.

We evaluate \sysname on hyperparameter tuning, single-server, and 
multi-server distributed training scenarios. We compare \sysname against
PyTorch using DALI. We use cloud servers specialized for machine
learning: 500 GB of DRAM, 24 CPU cores, 40Gbps Ethernet, eight GPUs
(V100/1080Ti) and either SSD or hard disk. We use the OpenImages
dataset~\cite{kuznetsova2018open, sarincrowdsource} for image
classification and FMA dataset~\cite{defferrard2016fma} for audio
classification.  For HP search on a single server with SSD, \sysname
accelerates training by 5.6\myx for the M5 audio model
~\cite{dai2017very} and 1.9\myx for ResNet50. On a single server with
SSDs and eight GPUs, \sysname accelerates training of models such as
ShuffleNet by up-to 1.8\myx.  For distributed training with 16 GPUs across two servers,
\sysname accelerates training AlexNet by 15\myx on hard drives, and
the M5 audio model training by 2.9\myx on SSDs.


The techniques in \sysname can
only help if the training is IO-bound or CPU-bound. If the model is GPU compute-intensive (e.g., language models such as Bert-L~\cite{devlin2018bert}),
IO and CPU may not be the bottleneck, thus leaving little for \sysname to do. 
Despite this
limitation, we show via extensive experimentation on a wide range of
DNN tasks, models, datasets, and hardware configurations that \sysname
significantly accelerates DNN training on commonly available ML optimized cloud servers.
The problem of data stalls will only worsen with time as
the size of data sets increase~\cite{training-big, abu2016youtube,
kuznetsova2018open} and GPUs become faster~\cite{rupp_cpu_nodate}.
%To aid in such predictive analysis while varying different parameters % (such as amount of DRAM, number of GPUs, etc.),
To help practitioners predict and analyze data stalls, 
we extend \tool to answer what-if questions about data stalls in DNN training (\eg What would be the impact on data stalls if GPU compute speeds increase by $2\times$?). 



%we believe \sysname will prove useful for accelerating
%training of many models. 
%\ap{Weak ending (last couple of lines).  I would roll this to the end of analysis para in intro (we find a large number of dnns \ldots).}

% contributions
In summary, this paper makes the following contributions:
\begincompactitemize
\item The first comprehensive analysis of how the data pipeline
  affects DNN training (\sref{sec-analysis})
\item The \tool tool for performing differential analyses and
  answering what-if questions about the impact of the data pipeline on
  DNN training (\sref{sec-tool})
%\item The novel partitioned caching, coordinated processing, and \minio
%  cache management techniques.
\item The design and implementation of the novel \sysname data loading
  library (\sref{sec-design})
 \item Evaluation showing the efficacy of \sysname in mitigating
 data stalls across a range of 3 tasks, 9 models, 4 datasets, and 
 2 different server configurations (\sref{sec-eval})
\end{itemize}


==> tables/tbl-analysis-cache-dist.tex <==

\begin{table}[!t]
  \small
  \centering
  \ra{1.1}
    \subfloat[Distributed training]{
   \begin{tabular}{c@{\hskip5pt}c@{\hskip5pt}}
  	\toprule[1pt]
  	Servers &  Storage IO (GB)\\
  	\midrule
  	1 & 125 \\
  	2 & 89  \\
  	3 & 48  \\
  	4 & 28  \\
  	\bottomrule[1pt]
  	%\subcaption{(a) Distributed training}
  \end{tabular}
  }
\quad
    \subfloat[HP Search]{
	\begin{tabular}{c@{\hskip5pt}c@{\hskip5pt}}
		\toprule[1pt]
		Jobs &  Storage IO (GB)\\
		\midrule
		1 x 8GPU & 125 \\
		2 x 4GPU & 258  \\
		4 x 2GPU & 467  \\
		8 x 1GPU & 884  \\
		\bottomrule[1pt]
		%\subcaption{(b) HP Search}
	\end{tabular}
	}
  
   \vspace{2pt}
    \mycaption{Storage IO per server}{This table shows the redundant storage IO incurred for distributed training and HP search}
\label{tbl-analysis-cache-dist}
\end{table}



==> tables/tbl-analysis-cache-hp.tex <==
\begin{table}[!t]
	\small
	\centering
	\ra{1.1}

	\begin{tabular}{c@{\hskip8pt}c@{\hskip8pt}c@{\hskip8pt}c@{\hskip8pt}c@{\hskip8pt}}
	\toprule[1pt]
	\# Jobs &  1x8GPU & 2x4GPU & 4x2GPU & 8x1GPU\\
	\midrule
	Storage \vio (GB) & 125 & 258 & 467 & 884 \\
	Read amplification & 1\myx & 2\myx & 3.7\myx & 7\myx \\
	\bottomrule[1pt]
	%\subcaption{(b) HP Search}
\end{tabular}
    \mycaption{Storage \vio in HP search}{This table shows the redundant storage IO incurred during HP search.}
\label{tbl-analysis-cache-hp}
\end{table}


==> tables/tbl-analysis-datastore.tex <==
\begin{comment}
	1GPU		4GPU		8GPU	
	ep1	ep3	ep1	ep3	ep1	ep3
local	1%	1%	24%	19%	53%	50%
blob	91%	1%	97%	19%	98%	50%
GFS	1%	1%	57%	51%	70%	60%
\end{comment}
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\begin{table}[!tbh]
  \small
  \centering
  \ra{1.3}
  \begin{tabular}{@{}l|rr|rr@{}}
	\toprule[1.2pt]
         Data store & \multicolumn{2}{c|}{4 GPU}  & \multicolumn{2}{c}{8 GPU} \\
                           & 1st Ep. & Stable Ep. & 1st Ep. & Stable Ep.  \\
          \midrule
          Local SSD & 24\% &  19\%	 &  53\%	& 50\% \\
	  Azure Blob & \textbf{97}\% &  19\%	 &  \textbf{98}\%	& 50\% \\
	  Gluster FS. & \textbf{57}\% &  \textbf{51}\%	 &  \textbf{70}\%	& \textbf{60}\% \\
  \bottomrule
   \end{tabular}
 \mycaption{Impact of data store on DNN training}{The table shows
       how the 1st and stabilized epoch time varies for 4 and 8 GPU 
       ResNet18 training job when different data stores
       are used for storing the dataset.}
       \vspace{-5mm}
\label{tbl-analysis-datastore}
\end{table}

==> tables/tbl-analysis-prep-hp.tex <==
%\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\setlength\mylength{\dimexpr.5\columnwidth-10\tabcolsep-0.5\arrayrulewidth\relax}

  	% Num jobs & 2 & 4 & 8 \\
  	%\emph{Prep Stall}  & 7\% & 25\% & 37\%  \\

\begin{table}[!t]
	\small
	\centering
	\ra{1.1}
	
	\begin{tabular}{c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c}
		\toprule[1pt]
		%\multicolumn{2}{c}{Models} & ShN & AN & RN18 & SqN & MN & RN50 & V11 \\
		Speed &  ShN & AN & RN18 & SqN & MN & RN50 & V11 \\
		\midrule
		3-CPU & 1731 & 1702 & 1242 & 927 & 824 & 726 & 778 \\
		24-CPU   & 3387 & 4437 & 2283 & 1461 & 1157 & 782 & 801 \\
		%Prep stall & 45\% & 47\% & 35\% & 33\% & 26\% & 17\% & 18\% \\
		\bottomrule[1pt]
	\end{tabular}
	
	\vspace{2pt}
	\mycaption{HP search with 8 jobs}{\small{(ShN-ShuffleNet, AN-AlexNet, RN18-Resnet18, SqN-SqueezeNet, MN-MobileNet, RN50-ResNet50, V11-VGG11)}}
	\label{tbl-analysis-prep-hp}
\end{table}





==> tables/tbl-analysis-preprocessing.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
  
 % \begin{tabular}{@{}lrrr@{}}
 \begin{tabular}{p{5em}*{3}{p{5em}}}
	\toprule[1.2pt]
	
	DNN & \multicolumn{3}{c}{Data Stall Time (for varying}\\
	& \multicolumn{3}{c}{\# of pre-processing threads)}\\
	& 8 & 16 & 24 \\
	\midrule
	VGG16 & 2\% & 2\% & 2\%  \\
	Resnet50 & 19\% & 2\% & 2\% \\
	Mobilenet & 68\% & 36\% & 30\% \\
	Squeezenet & 75\% & 47\% & 42\% \\
	Resnet18 & 76\% &  54\%& 50\% \\
	Shufflenet & 89\% & 81\%& 69\% \\
	Alexnet & 85\%  & 73\%& 64\%\\
	\bottomrule[1.2pt]
  \end{tabular}
  \vspace{2pt}

  \mycaption{Analysis of data stalls for various DNNs when the dataset is fully cached}{The table shows the impact of compute misses for seven different DNNs of varying computational complexities when trained using eight GPUs. The data pipeline cannot keep up with the ingest rate requirements for 8 GPUs, resulting in significant data stalls for most of the models under study.}
\label{tbl-analysis-preprocessing}
\end{table}


==> tables/tbl-analysis-summary.tex <==
\newcommand\VRule[1][\arrayrulewidth]{\vrule width #1}
\setlength{\tabcolsep}{3pt}
\begin{table*}[!t]
  \small
  \centering
     \vspace{-1em}
  \caption{Key findings and implications of our analysis of data stalls}
  \vspace{-1em}
  \ra{1.0}
 \begin{tabular}{!{\VRule[1pt]}m{0.435\textwidth}!{\VRule[1pt]}m{0.52\textwidth}!{\VRule[1pt]}}
	\specialrule{1.2pt}{0pt}{0pt}
	\rowcolor{grey} \centering
    \textbf{\emph{Finding}} & \Centering\textbf{\emph{\sysname Insights}}\\
    \specialrule{0.8pt}{0pt}{0pt}
    \rowcolor{white}
    OS Page Cache is inefficient for DNN training due to thrashing & Optimize DNN cache to eliminate thrashing across epochs (\textit{\minio} \sref{sec-minio})\\
    \specialrule{0.5pt}{0pt}{0pt}
    Lack of coordination among local caches lead to
    redundant \vio in distributed training across servers & Local caches of servers can be coordinated to fetch data from the remote cache to overcome storage \vio bottlenecks (\textit{Partitioned Cache} \sref{sec-part-cache}) \\
    \specialrule{0.5pt}{0pt}{0pt}
    No coordination in HP search leads to
    redundant \vio \& prep & HP search jobs must coordinate data fetch \& prep (\textit{Coordinated Prep} \sref{sec-coord-prep})\\
%    \specialrule{0.5pt}{0pt}{0pt}
%    DNNs need 3 -- 24 CPU cores per GPU for prep & Hardware must be upgraded carefully and in a balanced manner \\
%    \specialrule{0.5pt}{0pt}{0pt}
%    DNNs spend upto 65\% of epoch time in pre-processing data & We need optimized pre-processing libraries, or better data formats to speed up data augmentation.\\
	\specialrule{1.2pt}{0pt}{0pt}
   \end{tabular}
\label{tbl-analysis-summary}
\end{table*}



==> tables/tbl-dist-mint-net.tex <==

\begin{table}[!t]
  \small
  \centering
  \ra{1.1}
 \begin{tabular}{cccccc}
	\toprule[1pt]
	%Nodes  & 2 & 3 & 4 \\
	& \multicolumn{2}{c}{AlexNet (Mbps)} & \multicolumn{2}{c}{ResNet50 (Mbps)}\\
	Nodes & DALI & \sysname & DALI& \sysname \\
	\midrule
	2 & 0.59 & 13.92 & 1.02 & 5.45 \\
	3 & 0.66 & 14.08 & 1.11 & 5.69 \\
	4 & 0.66 & 15.09 & 1.18 & 5.76 \\
	%DALI (Gbps) & 0.59 & 0.66 & 0.66 \\
	%\sysname (Gbps) & 13.92 & 14.08 & 15.09 \\
	\bottomrule[1pt]
   \end{tabular}
%   \vspace{2pt}
    \mycaption{Network activity during co-ordinated caching}{}
\label{tbl-eval-net}
\end{table}



==> tables/tbl-eval-hp-cached-small.tex <==

\begin{table}[!t]
  \small
  \centering
  \ra{1.1}
  
   \begin{tabular}{c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c@{\hskip5pt}c}
  	\toprule[1pt]
  	%\multicolumn{2}{c}{Models} & ShN & AN & RN18 & SqN & MN & RN50 & V11 \\
  	Models &  ShN & AN & RN18 & SqN & MN & RN50 & V11 \\
  	\midrule
  	%Speed	&   DALI & 1441 & 1399 & 1056 & 835 & 752 & 569 & 552 \\
  	Speed & 1.8\myx & 1.9\myx & 1.5\myx & 1.5\myx & 1.4\myx & 1.2\myx & 1.2\myx \\
  	\bottomrule[1pt]
  \end{tabular}
  
   \vspace{2pt}
    \mycaption{HP search with \sysname on a fully cached dataset}{On \confssd, when training with the small ImageNet-1k dataset that fits in memory, \sysname provides upto 1.9\myx speedup by eliminating redundant pre-processing \small{(ShN-ShuffleNet, AN-AlexNet, RN18-Resnet18, SqN-SqueezeNet, MN-MobileNet, RN50-ResNet50, V11-VGG11)}}
\label{tbl-hp-cached-small}
\end{table}



==> tables/tbl-eval-storage-miss.tex <==
%\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newlength\mylengthnew
\setlength\mylengthnew{\dimexpr.5\columnwidth-10\tabcolsep-0.5\arrayrulewidth\relax}
\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
 \begin{tabular}{lrrrrr}
	\toprule[1pt]
         \textbf{\emph{Caching}} & 100\% & 70\% & 55\% & 35\% & 20\%\\
         \midrule
          \textbf{\emph{Page Cache}}  & 0\% & 46\% & 66\% & 84\%  & 97\% \\
           \textbf{\emph{\mint}}  & 0\% & 30\% & 47\% & 65\%  & 81\% \\
	\bottomrule[1pt]
   \end{tabular}
   \vspace{2pt}
    \mycaption{Storage Misses}{Percentage of storage miss in the page cache and \mint caching policy.}
    %(LRU policy) and the \mint caching policy. \mint results in 20\% lower storage misses on average compared to page cache. }
    \vspace{-2em}
\label{tbl-eval-storage-miss}

\end{table}



==> tables/tbl-gpu.tex <==

\begin{table}[!h]
  \small
  \centering
  \ra{1.3}
 \begin{tabular}{lrrrrr}
	\toprule[1pt]
	       \textbf{\emph{Num GPU}} & 1 & 2 & 4 & 8\\
	       \midrule
         \textbf{\emph{1080Ti}} & 0\% & 0\% & 0\% & 0\%\\
          \textbf{\emph{V100}}  & 53\% & 53\% & 53\% & 48\% \\
	\bottomrule[1pt]
   \end{tabular}
   \vspace{2pt}
    \caption{Pre-processing stall as a percentage of total training time .}
\label{tbl-hits}
\end{table}



==> tables/tbl-hits.tex <==
%\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}
\newlength\mylength
\setlength\mylength{\dimexpr.5\columnwidth-10\tabcolsep-0.5\arrayrulewidth\relax}
\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
  
   \begin{tabular}{lrrrr}
  	\toprule[1pt]
  	\textbf{\emph{Dataset cached (\%)}} & 100\% & 50\% & 35\% & 25\%\\
  	\midrule
  	\multicolumn{5}{l}{\textbf{\emph{Distributed 8-GPU training in a node}}}\\
  	\emph{Cache miss}  & 0\% & 71\% & 84\%  & 93\% \\
  	\emph{Ideal miss rate}  & 0\% & 50\% & 65\%  & 75\% \\

  	\midrule
  	\multicolumn{5}{l}{\textbf{\emph{8 HP search jobs in a node}}}\\
  	  	\emph{Disk IO (GB)}  & 0 & 642 & 750 & 884\\
  	  	\emph{Read amplification}  & 1\myx & 4.6\myx & 5.4\myx & 6.3\myx\\
  	\bottomrule[1pt]
  \end{tabular}
  
 %\subfloat[]{ 
 %\begin{tabular}{lrrrrr}
	%\toprule[1pt]
     %    \textbf{\emph{Caching}} & 100\% & 70\% & 55\% & 35\% & 20\%\\
      %    \textbf{\emph{Hit rate}}  & 100\% & 54\% & 34\% & 16\%  & 3\% \\
	%\bottomrule[1pt]
   %\end{tabular}
 %}
%\quad 
% \subfloat[]{ 
 %\begin{tabular}{lrrrrr}
%	\toprule[1pt]
%	\textbf{\emph{Caching}} & 100\% & 50\% & 35\% & 25\% \\
%%%	\bottomrule[1pt]
%\end{tabular}
% }
   \vspace{2pt}
    \caption{Percentage of page cache hits (LRU).\vc{Don't think this
        is adding a lot of value, we can simply say misses are 20\%
        higher than expected in single node case. Second table part is
      confusing at first, better explained directly in the text I think}}
\label{tbl-hits}
\end{table}



==> tables/tbl-ingestion-rate.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
  \begin{tabular}{@{}lrrrr@{}}
	\toprule[1.2pt]
	Task & \multicolumn{3}{c}{Expected Rate (in MBps)} & Data Pipeline \\
	Model \& & 1GPU & 4GPU & 8GPU & Rate (MBps)\\
	\midrule
    	\multicolumn{5}{@{}l}{\emph{Language Modelling (Wikipedia \& BookCorpus, 110GB)}}\\ 
	BERT-Large & 8 & 31 & 59 & 570 \\
	\midrule
	\multicolumn{5}{@{}l}{\emph{Language Translation (WNMT-16, 16GB)}} \\
	GNMT & 48 & 119  & 175 &  1047\\
   % \midrule
%	\multicolumn{5}{@{}l}{\emph{Image Classification (ImageNet, 140GB)}}\\
	
%	VGG16 & 24 & 83 & 170 & 327 \\
%	Resnet50 & 39 & 139 & 257 & 327 \\
%	Mobilenet & 99 & 308 & {\color{red}\textbf{484}} & 327 \\
%	Squeezenet & 119 & {\color{red}\textbf{377}} & {\color{red}\textbf{597}} & 327 \\
%	Resnet18 & 126 & {\color{red}\textbf{403}} & {\color{red}\textbf{626}} & 327 \\
%	Shufflenet & 298 & {\color{red}\textbf{791}} & {\color{red}\textbf{1048}} & 327 \\
%	Alexnet & {\color{red}\textbf{388}} & {\color{red}\textbf{793}} & {\color{red}\textbf{976}} & 327\\
%	\midrule
%	\multicolumn{5}{@{}l}{\emph{Object Detection (OpenImages, 310GB)}} \\
%	SSD & {\color{red}\textbf{85}} & {\color{red}\textbf{124}} & {\color{red}\textbf{164}} & 75 \\
	\bottomrule[1.2pt]
  \end{tabular}
%  \vspace{2pt}

  \mycaption{Data ingestion rate of language models}{The table enumerates
    the required data ingestion rate at the
    GPUs in MBps for two language tasks, and shows that their compute
    intensive nature results in GPU bound training.}
\label{tbl-ingestion-rate}
\end{table}


==> tables/tbl-mot.tex <==
\newcolumntype{P}[1]{>{\centering\arraybackslash}p{#1}}

\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
  
  \subfloat[]{
  \begin{tabular}{@{}lr@{}}
	\toprule[1.2pt]
    Model & Data \\
    		& Stall \\
	\midrule
    MobileN. & 29\% \\
    SqueezeN. & 37\% \\
    ResN.18 & 50\% \\
    AlexN. & 65\% \\
    ShuffleN. & 65\% \\
	\bottomrule[1.2pt]
    %\subcaption{(a)}
  \end{tabular}
}
\quad
    \subfloat[]{
    \begin{tabular}{@{}cp{0.5cm}@{}}
    \toprule[1.2pt]
      \# 1-GPU & Data\\
      Jobs & Stall \\
    \midrule
      1 & 1\% \\
      2 & 14\% \\
      4 & 30\% \\
      6 & 42\% \\
      8 & 53\% \\
    \bottomrule[1.2pt]
      %\subcaption{(a)}
    \end{tabular}
  }
  \quad
    \subfloat[]{
    \begin{tabular}{@{}cr@{}}
      \toprule[1.2pt]
        Percent  & Epoch  \\
          Cached & Time (s) \\
      \midrule
      100\% & 271 \\
      75\% & 1629 (6\myx) \\
      50\% & 3258 (12\myx) \\
      25\% & 4887 (18\myx) \\
      0\% & 6516 (24\myx) \\
    \bottomrule[1.2pt]
      %\subcaption{(b)}
    \end{tabular}
  }

  \vspace{-3mm} \mycaption{Data Stalls}{ Table (a) lists the
    percentage of time in each epoch spent handling data stalls for
    different DNN models running on eight V100 GPUs (dataset is fully
    cached). Table (b) lists the data stall overhead when concurrent ResNet18
    hyperparameter search jobs (each using a single GPU) are running
    on the same machine (dataset is fully cached). Table (c) lists the
    per-epoch training time when the dataset is partially cached for
    ResNet18 model running on eight GPUs.  Even when data is fully
    cached, pre-processing data leads to overheads as high as
    65\%. When only 25\% of the data set is cached, training time
    increases by 18\myx as data has to be fetched from hard drives.}
    %Data stalls form a significant portion of overall training time for many models.
\label{tbl-mot}
\jm{This table is up to date (DALI). The hard drive numbers for x\% caching assumes x\% hit rate.}
\vspace{-5mm}
\end{table}


==> tables/tbl-pp-hit.tex <==

\begin{table}[!t]
  \small
  \centering
  \ra{1.3}
 \begin{tabular}{llllll}
	\toprule[1pt]
	    \textbf{\emph{Num jobs per node}} & 2 & 4 & 8 \\
	    \midrule
         \textbf{\emph{Current pre-proc miss}} & 100\% & 100\% & 100\%\\
          \textbf{\emph{Ideal miss rate}}  & 50\% & 25\% & 12.5\% \\
	\bottomrule[1pt]
   \end{tabular}
   \vspace{2pt}
    \caption{Prep miss rate}
\label{tbl-prep-miss}
\end{table}



==> tables/tbl-sku.tex <==

\begin{table}[!h]
  \small
  \centering
  \ra{1.3}
 \begin{tabular}{cccccccc}
	\toprule[1pt]
	     \textbf{\emph{}} & GPU model & GPU count & GPU DRAM (GB) & CPU cores & DRAM (GB) & Storage & Rand Read Thr (MBps)\\ 
         \textbf{\emph{SKU1}} & V100 & 8 & 32 & 28 & 500 & SSD & 530 \\
          \textbf{\emph{SKU2}} & 1080Ti & 8 & 11 & 28 & 500 & HDD & 15 -- 50 \\
	\bottomrule[1pt]
   \end{tabular}
   \vspace{2pt}
    \caption{Percentage of page cache hits (LRU).}
\label{tbl-hits}
\end{table}



==> tables/tbl-tensorflow-small.tex <==
\setlength\mylength{\dimexpr.5\columnwidth-10\tabcolsep-0.5\arrayrulewidth\relax}
\begin{table}[!t]
    \small
 	\centering
 	\ra{0.9}
 	
 	  \begin{tabular}{@{}c|c|cc@{}}
 		\toprule[1.2pt]
 		%      & \multicolumn{3}{c}{\% dataset cached}\\
 		\% dataset cached  &   8-GPU training & \multicolumn{2}{c}{8-job HP search}\\
 			(Size : 146GB) &  Cache Miss	   &   Disk IO (GB) & Read amp \\
 		\midrule
 		50\% & 91\% & 860 &  6.14\myx \\
 		35\% & 94\% & 1010 & 7.21\myx \\
 		25\% & 97\% &  1019 & 7.28\myx \\
 		\bottomrule[1.2pt]
 	\end{tabular}
 	%\vspace{-1em}
    \mycaption{Data stalls in Tensorflow}{The fundamental problems that result in data stalls-inefficient caching and thrashing due to lack of coordination in HP search, exist in TF.}
\label{tbl-analysis-tf-small}
	\vspace{-3em}
\end{table}



==> tables/tbl-tensorflow.tex <==

\begin{table}[!h]
    \small
 	\centering
 	\ra{1.3}
 	
 	  \begin{tabular}{@{}llll@{}}
 		\toprule[1.2pt]
 		      & \multicolumn{3}{c}{\% dataset cached}\\
 		Dataset (140GB)      & 50\% & 35\% & 25\% \\
 		\midrule
 		\multicolumn{4}{l}{\emph{8 GPU training}}\\ 
 		Observed Cache miss & 91\% & 94\% & 97\% \\
 		Expected Cache miss & 50\% & 65\% & 75\%\\
 		\midrule
 		\multicolumn{4}{l}{\emph{8 job HP search}} \\
 		Observed Time(s) & 1710 &  2073 & 2176\\
 		Expected Time(s) &1148 &  1148 & 1150 \\
 		Disk fetch (GB)  &860 & 1010  & 1019 \\
 		Read amplification & 6.14\myx & 7.21\myx & 7.28\myx \\
 	
 		\bottomrule[1.2pt]
 	\end{tabular}
 	
 	
 %	\setlength{\tabcolsep}{2pt}
 %	\subfloat[]{
 %		\begin{tabular}{@{}lr@{}}
 %			\toprule[1.2pt]
 %			\multicolumn{2}{l}{Cache Miss Rate} \\
 %			\midrule
%			Observed & 85\% \\
%			Expected & 35\% \\
 %			\bottomrule[1.2pt]
 %			%\subcaption{(a)}
 %		\end{tabular}
 %	}
 %	\qquad
 %	 	\subfloat[]{
 %		\begin{tabular}{@{}lr@{}}
 %			\toprule[1.2pt]
 %			 \multicolumn{2}{l}{HP search time (s)} \\
 %			 \midrule
 %			Observed & 2073 \\
 %			Expected & 1150 \\
 %			\bottomrule[1.2pt]
 %			%\subcaption{(a)}
 %		\end{tabular}
 %	}

    \caption{Tensorflow data stall analysis}
\label{tbl-analysis-tf}
\vspace{-2em}
\end{table}



==> tables/tbl-tool.tex <==

\begin{table}[!t]
  \small
  \centering
  \ra{1.1}
 \begin{tabular}{ccccc}
	\toprule[1pt] 
	 \% dataset cached $(x)$ & 25\% & 35\% & 50\% \\% & 100\% \\
	     \midrule
         \emph{$F_{predicted}$} & 6226 & 7164 & 9225 \\%& 9727  \\
         \emph{$F_{empirical}$} & 6130 & 7118 & 9022 \\%& 9484 \\
	\bottomrule[1pt]
   \end{tabular}
%   \vspace{2pt}
    \caption{Training speed (samples/s) predicted by the \tool is atmost
    4\% different from empirical values.}
\label{tbl-tool}
\end{table}



==> v3/background.tex <==
\section{Background}
\label{sec-bkgd}


%\input{fig-dali/fig-processing-rate-res18}

Deep Neural Networks (DNNs) are a class of ML models that
automatically extract higher level features from the input data.  The
DNN is trained over multiple rounds termed \emph{epochs}. Each epoch
processes all items in the dataset exactly once, and consists of
multiple \emph{iterations}; each iteration processes a random,
disjoint subset of the data termed a \emph{minibatch}. The DNN is
trained until a target accuracy is reached. Training a DNN model to reach a
given accuracy consists of two steps: %(i) finding the optimal set of
%hyperparameters for the learning process, and (ii) running the learning
%algorithm until the desired accuracy is reached. 
\vspace{-0.5em}
\begin{enumerate}[leftmargin=18pt]
\itemsep0em 
\item \vheading{Hyperparameter (HP) search}. There are many parameters for
the learning algorithm that must be provided before the start of
training.  These hyperparameters (for \eg learning rate, its decay,
dropout, and momentum) influence the speed and quality of
learning.  %Examples of hyperparameters are learning rate, its decay,
%dropout, and momentum.  
During the search process, we start several
training jobs; each job trains the model with different
hyperparameters, on each available GPU (or a distributed job across
several GPUs); progress is checked after a few epochs and the
worst-performing candidates are killed and replaced by new jobs with
different hyperparameters that are chosen
algorithmically~\cite{bergstra2012random, jaderberg2017population,
  golovin2017google, hyperband}.
% , chosen using algorithms like Random
% Search~\cite{bergstra2012random}, Population Based
% Training~\cite{jaderberg2017population}, Median Stopping
% Rule~\cite{golovin2017google}, or Hyperband~\cite{hyperband}.
Tuning
hyperparameters is crucial for generating DNN models that have high
accuracy~\cite{hyper-importance}.

\item \vheading{Training the model to target accuracy}.
%Once the
%hyperparameters have been decided,
The second step is to obtain models
with high accuracy by training it with input data, using the
hyperparameters chosen in the previous step.
\end{enumerate}

\subsection{The DNN ETL Requirements}
\label{sec-etl}
In every epoch of training, the input dataset 
is subjected to a ETL (extract-transform-load) before being processed at the GPU
(or any other accelerator). 
\revision{The ETL process in the data pipeline of popular image-based DNN training} imposes several unique data 
ordering constraints to ensure model convergence and achieve state-of-the-art accuracy. 
\vspace{-0.5em}
\begin{itemize}[leftmargin=18pt]
	\item The dataset must be shuffled every epoch to ensure the order in which data 
	items are accessed are random in each epoch %(\emph{Ordering invariant})
	\item An epoch must use \emph{all} data items in the dataset \emph{exactly} once %(\emph{Frequency invariant})
	\item In every epoch, the data transformations(pre-processing) must be random; the same transformed item should not be used across epochs
	%(\emph{Transformation invariant}).
\end{itemize}
\revision{Several prior work have theoretically and empirically demonstrated that
relaxing these constraints will affect the convergence rate of 
SGD~\cite{convergence, chung2017ubershuffle, localsgd, perez2017effectiveness}.
While some NLP and recommendation models may not require random pre-processing and data 
shuffling every epoch, the focus of our work is computer vision and audio models
where random data augmentation and shuffling is the default and common practice~\cite{mlperf-train,
pytorch-ex}.
Therefore, in this work, all our experiments abide by the aforementioned ETL 
requirements.}

\subsection{DALI : Fast Data Pipelining} State-of-the-art data loading
and pre-processing libraries like DALI can be used as a drop in
replacement for the default dataloaders in frameworks like PyTorch,
TensorFlow, or MxNet. DALI can accelerate data pre-processing
operations %on Nvidia GPUs using the \texttt{NVJpeg} image decoding
%library, and by 
using GPU-accelerated data pre-processing operations. DALI
also \emph{prefetches and pipelines} the data fetch and pre-processing with
the GPU compute, similar to the default dataloader in PyTorch. We empirically
verified that DALI outperforms the default data pipelines of PyTorch, TensorFlow, 
and MxNet. Therefore, throughout this work, unless and otherwise stated,
we use DALI, as it is the strongest baseline.


\section{Data Stalls in DNN Training}
\label{sec-data-stalls}
We now discuss our formulation of data stalls.
% and illustrate it with an example.
Consider the training process of a typical DNN. It
executes the following steps in each iteration of an epoch:
\begin{enumerate}[leftmargin=18pt]
	\itemsep0em 
	\item A minibatch of data items is fetched from storage.
	\item The data items are pre-processed, for \eg, for image classification, data items are decompressed, and then randomly cropped, resized, and flipped.
	\item The minibatch is then processed at the GPU to obtain the
	model's prediction %(\emph{forward pass}).
	\item A loss function is used to determine how much the prediction
	deviates from the right answer%; both weight an activation gradients
	%are computed across the different layers of the DNN 
	%(\emph{backwardpass}).
	%\item Weights in the model's layers are updated using gradients computed %in 
	%the backward pass %(\emph{weight update}).
	\item Model weights are updated using computed gradients
	
\end{enumerate}

\input{fig-analysis/fig-rates}

Ideally, most of the time in each epoch should be spent on Steps 3--5
(which we collectively term the \textit{GPU compute} time), i.e.,
training is \emph{GPU bound}. When performing multi-GPU training,
individual GPUs (workers) exchange weight gradients with other workers
before performing weight update.  For this work, we
roll the communication time for gradient exchange during multi-GPU
training into computation time. 

In most frameworks including PyTorch, TensorFlow, and MxNet,
data preparation (Steps 1 and 2) and GPU computation execute in a
pipelined fashion; i.e., subsequent minibatches are \emph{prefetched and
	pre-processed} by data preparation threads, using multiple CPU cores on
the machine, as the GPU computes on the current minibatch of data.  If
the GPU is waiting for Steps 1--2 to happen, we term it a \emph{data
	stall}. Specifically, if training is blocked on Step 1, we call it a
fetch stall; the training is \emph{I/O bound} in this case.  Training
blocked due to Step 2 is termed prep stall; this causes the training
to be \emph{CPU bound}.  Data stalls cause the GPU to be idle, and
must be minimized to increase GPU utilization. 

The rate at which data items can be fetched from storage (Step 1)
depends primarily on the storage media. The rate at which data items
can be pre-processed (Step 2) depends upon the pre-processing
operations and the number of CPU cores available for pre-processing.


In general, if we prefetch data at rate $F$, 
pre-process it at rate $P$ and perform GPU computation
on it at rate $G$, then data stalls appear if $G > min(F, P)$, i.e.,
GPU processes data at a rate faster than it can be prefetched or 
pre-processed. 

Any fetch or prep stall implies idle GPU time, which must be minimized.
The fetch and prep stalls reported in this work
are unmasked
% fetch and prep time respectively;
stall time;
i.e.,
the
%amount of
stall time that shows up in the critical path,
inspite of being pipelined with compute. From now on, we call data prefetching simply \emph{fetch},
and pre-processing \emph{prep}.








==> v3/eval.tex <==
\section{Evaluation}
\label{sec-eval}

We now evaluate the efficacy of \sysname on three different
aspects of the training process:  multi-GPU
training on a single server, distributed training across multiple
servers, and hyperparameter tuning.  We evaluate our techniques on \textbf{nine} models,
performing \textbf{three} different ML tasks (image classification,
object detection and audio classification) on four different
datasets, each over 500GB as shown in Table~\ref{tbl-dataset-models}.
Since DALI strictly outperforms PyTorch DL, we use 
DALI as the baseline in our experiments. 
For each model, we run both CPU-based (all pre-processing on CPU) 
and GPU-based (part of decoding and all other transformations on GPU)
 mode of DALI, and present the best of the two results.




\vheading{Experimental setup}.  We evaluate \sysname on two
representative server configurations from Microsoft clusters
  as described in Table~\ref{tbl-analysis-sku}. %each with 500 \gb DRAM, 24 CPU cores, 40 Gbps Ethernet, eight GPUs, and 1.8 \tb of storage space.
 \confssd uses V100 GPUs and a SATA SSD, while \confhdd uses
1080Ti GPUs and a magnetic hard drive. 
%\confssd is similar to the AWS
%\texttt{p3.16xlarge} instance~\cite{aws-p3}, while \confhdd is similar
%to the AWS \texttt{p2.8xlarge} instance~\cite{aws-p2}. 
We use the same training methodology we used for analysis (\sref{sec-methodology}).
We seek to answer the following questions:

\input{tables/tbl-evalq}


\input{fig-dali/eval}

\subsection{Single-server Multi-GPU training}
\label{sec-mint}

\sysname speeds up a single-server training job by reducing cache
misses using the \minio cache. Figure~\ref{fig-eval} (a) plots the
relative speedup with respect to DALI while training the image
classification and object detection models on the OpenImages dataset,
and audio classification on FMA dataset. We evaluate \minio against
two modes of DALI. DALI's default mode is \emph{DALI-seq}, where it
reads data sequentially off storage and shuffles them in
memory~\cite{dali-shuffle}. \emph{DALI-shuffle} accesses the dataset
in a randomized order (doing random reads, similar to the native dataloader of PyTorch).


\minio results in upto 1.8\myx higher training speed
compared to DALI-seq by eliminating thrashing on \confssd. When the
image classification models are trained with ImageNet-22k dataset,
\sysname results in up to 1.5\myx speedup. \sysname
accelerates ResNet50 training on 
OpenImages by 2.1\myx compared to DALI-seq and 1.53\myx 
compared to DALI-shuffle on \confhdd.

 
\vheading{Reduction in cache misses}. We measure the disk \vio and
number of cache misses when training ShuffleNet on OpenImages dataset
on \confssd. This server can cache 65\% of the dataset. \sysname
reduces misses to the minimum number of 35\%, resulting in 225 GB of
\vio. In contrast, DALI-Seq results in 66\% cache misses, increasing
\vio by 87\% to 422 GB; DALI-shuffle results in 53\% cache misses,
increasing \vio by 50\% compared to \sysname to 340 GB.


%\input{tables/tbl-eval-fetch-miss}
 
Note that, when the whole dataset does not fit in memory, DALI-shuffle
performs better than DALI-seq (because sequential access is a
pathological case for the Linux LRU page cache). 
Therefore, our
evaluation in the rest of this section compares \sysname to the
stronger baseline, DALI-shuffle.

\vspace{-1em}
\subsection{Multi-Server Distributed Training}
\label{sec-dist-mint}
We now evaluate \sysname on a distributed training scenario.
%As discussed in \sref{sec-design},
The lack of cache co-ordination between the participating servers
results in fetch misses that lead to disk I/O.  \sysname uses
partitioned caching to avoid redundant \vio.
Figure~\ref{fig-eval}(b) shows that \sysname improves the throughput
of distributed training jobs by upto 15\myx (AlexNet on OpenImages)
when trained across two servers on \confhdd(16 GPUs). On \confhdd
servers, 65\% of the OpenImages dataset can be cached on a single
server; and it can be fully cached in the aggregated memory of two
servers. Therefore, \sysname moves the training job from being I/O
bound to GPU bound.
When trained across two servers on \confssd, \sysname accelerates
ShuffleNet on ImageNet-22k by 1.3\myx, and Audio-M5 on FMA by 2.9\myx.
On \confssd, the relative gains are lower because the cost of a fetch
miss is lower on SSDs due to its high random read throughput, as
compared to HDDs on \confhdd.



\input{fig-dali/fig-eval-2}


\subsection{Hyperparameter Search}
\label{sec-unified}


Figure~\ref{fig-eval} (d) plots the relative increase in throughput of
individual jobs across several models when eight concurrent HP search
jobs are run on a \confssd server. On less computationally complex
models like AlexNet and ShuffleNet, \sysname increases training speed
by 3\myx, because these models are originally CPU bound due to prep.
%the expensive pre-processing operations.
For the audio model, \sysname increases the training speed by
5.6\myx. \sysname reduced the total disk \vio from 3.5TB to 550GB. %,
Similarly, on \confhdd, \sysname results in 5.3\myx faster training on
the audio model, and 4.5\myx faster training on ResNet50.
On \confhdd, \sysname results in 5.3\myx
faster training on the audio model, and 4.5\myx faster training on
ResNet50 by coordinating data fetch and prep.


\vheading{Split of coordinated prep benefits}.
Next, we show the breakdown of speedup due to coordination
of data fetch and prep during HP search.
When fetch is coordinated, concurrent jobs use data fetched by other jobs; but each job performs its own data prep. 
\sysname coordinates both; eliminating redundant fetch and prep.
Figure~\ref{fig-eval} (e) plots the results on \confssd. 
In this case, data stall is dominated by 
prep, which \sysname mitigates %using coordinated prep 
unlike prior work like Quiver~\cite{kumar2020quiver} that only coordinates fetch.
%Coordinating data fetch only solves a small part of the data stalls.

%\vspace{-0.5em}
\vheading{Multi-GPU HP search jobs}.  Figure~\ref{fig-eval} (f)
%evaluates the efficacy of \sysname for different configurations
%of 
shows training with different configs of HP search jobs on a machine; 8 1-GPU jobs, 4 2-GPU jobs, 2
4-GPU jobs, or 1 8-GPU job for AlexNet on OpenImages. For a single job
case, the benefit is due to the \minio cache; in other configs,
it is due to coordinated prep. More the number of concurrent jobs, higher the benefit
with coordination.



\vspace{-0.2em}
\subsection{Training to Accuracy with \sysname}
\label{sec-eval-accuracy}
\vspace{-0.2em}
\sysname does not change the randomness of data pre-processing
 involved. Its techniques do not affect the learning algorithm.
To demonstrate this, we train ResNet50 to accuracy on ImageNet-1K
using 16 GPUs across two \confhdd servers, where each server is
capable of caching 50\% of the dataset.
Figure~\ref{fig-accuracy} shows that \sysname reduces the time to
target accuracy (75.9\%) from two days to just 12 hours (4\myx
better), due to partitioned caching.



\subsection {Resource Utilization}
\label{sec-resource}
\vspace{-0.5em}
\vheading{\minio results in lower disk I/O and better CPU utilization}.
Figure~\ref{fig-mint-io} shows the I/O for two epochs of training
ResNet18 on OpenImages on \confssd.  The I/O behavior is similar
across models and server configurations.
DALI observes cache hits at the beginning of the epoch, but
soon becomes I/O bound.% (disk bandwidth: 530 MB/s).

Since \minio is caching a random subset of the dataset, 
%However, due to \minio's no replacement policy,
cache hits are uniformly distributed across the epoch in
\sysname. This results in a predictable I/O access pattern and faster
training (epochs end earlier in Figure~\ref{fig-mint-io}).
Profiling the CPU during training shows that the prep
threads in DALI are often stalled waiting for I/O. Since \minio
reduces the total disk I/O, \sysname is able to better utilize the CPU
for pre-processing. The combination of lower disk I/O and
better CPU utilization leads to shorter training time in \sysname.


\vheading{\sysname uses a fraction of available network
  bandwidth}. \sysname shards the dataset equally among all servers in
distributed training to ensure load balancing. We track the network
activity during the distributed training for ResNet50 on OpenImages
across two, three, and four servers with DALI and \sysname. \sysname
used 5.7 Gbps per server of network bandwidth (14\% of the 40 Gbps
available). DALI used 1.18 Gbps  of network
bandwidth per server. \sysname used 4.8\myx higher network bandwidth to train
4.3\myx faster.% than DALI.



\vheading{Coordinated prep has low memory overhead}.  %By design,
%co-ordinated prep has the same memory requirements as DALI. %To
%experimentally validate this, 
We track the memory utilization of
running hyperparameter search on AlexNet on OpenImages on \confssd using eight concurrent jobs.
\sysname uses 5 GB of extra process memory to store prepared
mini-batches in memory until all hyperparameter jobs consume it. We reduce the cache space given to \sysname by 5 GB (keeping the total
memory same for \sysname and DALI). Despite the lower
cache space, \sysname still accelerated training by 2.9\myx.


\vspace{-0.5em}
\subsection{\sysname on DGX-2}
\label{sec-dgx2}
\vspace{-0.1em}
%\input{fig-dali/fig-dgx2}
We now compare \sysname against DALI on the bleeding-edge
ML optimized server DGX-2 while performing HP search 
across 16 GPUs using OpenImages dataset. 
Since this dataset can be fully cached in the memory of
DGX-2 (1.5TB DRAM), we observe no stalls due to data fetch beyond
the first epoch. However, the imbalance in the ratio of CPU-GPU 
results in prep stalls which \sysname mitigates by coordinating
pre-processing.  
\sysname accelerates HP search by 1.5\myx -- 2.5\myx over DALI
by eliminating redundant data prep, enabling efficient usage of CPU
to mask prep stalls. 




==> v3/intro.tex <==
\section{Introduction}
\label{sec-intro}


% ML and DNN together. Throw some data too
Data is the fuel powering machine learning~\cite{andrew-ng}. 
Large training datasets are empowering state-of-the-art accuracy
for several machine learning tasks. Particularly, Deep Neural Networks (DNNs), have gained
prominence, as they allow us to tackle problems that were previously
intractable, such as image
classification~\cite{krizhevsky2012imagenet,simonyan2014very,he2016deep},
translation~\cite{wu2016google}, speech
recognition\cite{graves2013speech}, video
captioning~\cite{venugopalan2015sequence}, and even predictive
health-care~\cite{deepmind-health}.


Empowering DNNs to push state-of-the-art accuracy requires the model to
be trained with a large volume of data.
 During training, the model predicts the output given training data; based on
the output, the model's weights are tuned. This happens iteratively,
in many rounds called epochs. 
\begin{comment}
The training process uses configuration
options called hyperparameters (HP) that influence the speed and
quality of the learning process. So the first step in training a model
is finding the optimal set of HP. HP search is typically performed by
launching several parallel jobs with different hyperparameters,
monitoring their progress, and replacing poorly performing ones with
new values, until the best hyperparameters are found. 
 Once the hyperparameters are decided, DNN training is performed on a single
GPU, single server with multiple GPUs, or across multiple servers.
\end{comment}

However, DNN training is data-hungry, resource-intensive, and
time-consuming. It involves the holistic use of all
the resources in a server from storage and CPU for 
fetching and pre-processing the dataset to the GPUs that perform 
computation on the transformed data. 
Researchers have tackled how to efficiently use these
resources to reduce DNN training time,
%Researchers have tackled reducing DNN training time using a number of
%different approaches
such as reducing communication
overhead~\cite{lin2017dgc, PoseidonATC2017, hashemi2018tictac,
	jayarajan2019priority, narayanan2019pipedream}, GPU memory
optimizations~\cite{vdnn,chen2016training, gist2018}, and
compiler-based operator optimizations~\cite{vasilache2018tensor,
	chen2018tvm,jia2019taso}.
%However, the impact of the \emph{data
% pipeline} on DNN training has been relatively unexplored.
However, the impact of storage systems, specifically the \emph{data
	pipeline}, on DNN training has been relatively unexplored.


\input{tables/tbl-summary}


\vheading{The DNN Data Pipeline}. 
During DNN training, the data pipeline works as follows. Data items
are first fetched from storage and then \emph{pre-processed} in memory. 
For example, for many important and widely-used
classes of DNNs \revision{in computer vision}, there are
several pre-processing steps: data is first decompressed,
and then random perturbations such as cropping the image or rotating
it are performed to improve the model's
accuracy~\cite{perez2017effectiveness}. Once pre-processed, the data items
are sent to the GPUs for processing. One complete pass over the training 
dataset is termed an epoch; models are iteratively trained for several epochs to 
achieve desired accuracy.

The DNN data pipeline operates in parallel with GPU computation. Ideally, the data pipeline should steadily feed 
pre-processed data items to the GPUs to keep them continuously busy
processing data; we term this GPU-bound. Unfortunately, training
\revision{image, video, or audio models} is often \vio-bound, bottlenecked by fetching the data from storage, or
CPU-bound, bottlenecked by applying data pre-processsing in
memory. Collectively, we term these bottlenecks \textbf{data stalls} and
differentiate between \emph{prep stalls} (time spent on data pre-processing)
and \emph{fetch stalls} (time spent on \vio).

\begin{comment}
\vheading{Novelty over prior work}. Recent work like
Quiver~\cite{kumar2020quiver} demonstrate how to speed up DNN
training by efficiently caching data from remote object store on local
storage. In contrast, %our work shows that most publicly available, large datasets can fit on local storage and the overhead of remote fetch is amortized by training for several epochs (\sref{sec-fetch-remote}). O
our  work  assumes as baseline the setting where all data is
available on local storage (as most publicly available datasets for popular models fit on local storage~\cite{training-big,
	abu2016youtube, kuznetsova2018open, defferrard2016fma, imagenet-22k, russakovsky2015imagenet}, \sref{sec-fetch-remote}), and shows how to further
optimize the data pipeline (\sref{sec-fetch}, \sref{sec-prep}). This work therefore fundamentally improves performance on top of what Quiver can achieve.  While prior work like
Cerebro~\cite{cerebro}, and DeepIO~\cite{zhu2018entropy} have looked
at optimizing data fetch in distributed training, they do not
systematically analyze data stalls in different training scenarios, or
demonstrate how to accelerate single-server training.
\end{comment}

%\vspace{-1.5em}
% the contributions para
\subsection{ Contributions}

\vheading{Categorizing, measuring, and analyzing data stalls}.
We present the first comprehensive analysis
of data stalls (categorized as fetch and prep stalls) in DNN training.
We analyze nine popular DNN models from three domains
\revision{(image classification, object detection, and audio classification)} and
four datasets in a production cluster at Microsoft.
We vary factors such as the storage media, amount of data that can be cached in memory, the number of
CPU threads used to fetch and pre-process data,
and GPU generation.  We then analyze how these factors affect the data
pipeline and DNN training. \revision{Our analysis shows that data stalls are prominent in
popular computer vision and audio DNNs, as opposed to text-based NLP models.} Our analysis finds that data stalls squander away 
the improved performance of faster GPUs, even on ML optimized servers 
like the DGX-2~\cite{dgx2}.
Revisiting the insights from Stonebraker \etal~\cite{stonebraker81},
our analysis corroborates that relying on OS abstractions (like Page Cache)
is inefficient for DNN workloads. We also find that the data pipelines in popular
training frameworks like PyTorch and TensorFlow are inefficient in their
use of CPU and memory resources,
despite using state-of-the-art data-loading libraries like
DALI~\cite{noauthor_fast_2019} that reduce prep stalls using
GPU-accelerated data pre-processing. 
Table~\ref{tbl-summary}
summarizes the findings and insights of our analysis.
%DALI intro moved to background


\vheading{Performing predictive what-if analysis of data stalls}.
Performing an analysis of how the data pipeline impacts DNN training
is challenging since DNN training has a high degree of concurrency; it
is hard to isolate the time taken to perform a single task
as data pre-processing is pipelined with GPU
computation.  We develop a tool, \tool, that uses differential
analysis between runs (\eg comparing a run where data is completely
cached vs when data needs to be fetched from storage) to 
identify data-stall bottlenecks. Using the measured data stalls, it
answers what-if questions to help practitioners predict and analyze
data stalls (\eg What would be the impact on data stalls if DRAM
capacity increased by $2\times$?).

\setlength{\skip\footins}{0.5pc plus 5pt minus 5pt}
\vheading{Mitigating data stalls}. We use the insights from our
analysis to identify opportunities for improvement. We build a new
Coordinated Data Loader, \sysname \footnote{Read as cordial},%, that does not require any changes to the cluster infrastructure. 
that uses three main techniques to
mitigate data stalls. First, inspired by the pioneering work of
Stonebraker \etal on database caching~\cite{stonebraker81}, we demonstrate
that relying on the OS page cache is sub-optimal for DNN training.  We
implement \minio, a software cache that is specialized for DNN training.
%This cache exploits the unique data access
%pattern in DNN training to minimize the amount of data fetched from
%storage for training on a single server.
Second, we describe the \emph{partitioned caching} technique to coordinate
the \minio caches of servers involved in distributed training over
commodity network stack.  Third, we discuss the \emph{coordinated prep}
technique to carefully eliminate redundancy in data prep among
concurrent hyperparameter  search jobs in a server. We implement these
techniques as part of the user-space library \sysname, built on top of
the state-of-the-art data pipeline DALI~\cite{noauthor_fast_2019}.  We
evaluate \sysname across different models, datasets, and hardware and
show that it can accelerate training by up-to 5\myx on a single server
by mitigating data stalls over DALI.

%\vheading{Future research directions}. Our analysis
% fuels interesting research questions 
%with regards to mitigating data stalls. Most notably, 
%we observe the need for a
%GPU-CPU co-designed data transformation library for DNN
%training that automatically splits transformation operations 
%across available resources to ensure maximum utilization and
%minimize GPU idle time. 



==> v3/related.tex <==
\section{Related Work}
\label{sec-related}
%\vspace{-0.3em}
To the best of our knowledge, this paper presents the first comprehensive
analysis of data stalls in DNN training. %We place our work in the
%context of prior work.

\vheading{Optimizing remote storage via local
  caching}. Quiver~\cite{kumar2020quiver} uses local SSD caches to
eliminate the impact of slow reads from remote storage. The best case
for Quiver is when the dataset is completely cached on local storage;
our system starts from this baseline and further improves
performance. Quiver does not consider or optimize prep stalls, only
handling fetch stalls. 

%Since we talk about it in intro, skipping this

\vheading{Partitioned caching}.  Cerebro~\cite{cerebro} uses a
new parallel SGD strategy for model selection tasks. It partitions the
dataset across the servers in a cluster and hops the models from one
server to other, instead of shuffling
data. %, to minimize data fetch overhead.
Cerebro does not improve DNN training on a single
server, while \sysname optimizes performance in this scenario.
Furthermore, Cerebro is designed specifically for distributed
model search; on the contrary, our analysis and \sysname have a
broader scope.  DeepIO~\cite{zhu2018entropy} uses a partitioned
caching technique for distributed training with remote data, but
relies on specialized hardware like RDMA. In contrast, our work shows
that it is possible to mask fetch stalls using commodity TCP
stacks. %While prior work ~\cite{cerebro, zhu2018entropy} have looked at optimizing data fetch in distributed training, they do not systematically analyze data stalls in different training scenarios, or demonstrate how to accelerate single-server training.

%, with no changes to cluster infrastructure.
%In summary, none of these works analyze or mitigate data stalls in a single server training scenario, which our work addresses.

%All these works need changes to the cluster infrastructure to support a cache manager, scheduler, or new hardware, and cannot 
%eliminate data stalls in single-server training. 
%In contrast, \sysname does not need infrastructure changes, is entirely 
%implemented in a library used by individual training jobs and can accelerate single-server training by mitigating data stalls.

%new Prior work like DeepIO~\cite{zhu2018entropy} and 
%Cerebro~\cite{cerebro} have explored the use of cache partitioning for 
%distributed DNN training with remote storage. However, they either assume 
%a simplistic data pipeline that violates some ETL requirements considered 
%in this work~\cite{cerebro}, or require specialized hardware support like RDMA~\cite{zhu2018entropy}.
%Our work adds to the observations made by prior work on two fronts; that data stalls
%are prominent even when dataset is local or cached in memory, and the need for
%DNN-aware in-memory caching and redundancy elimination techniques.


%looked at distributed caching techniques.% for specific DNN training
%settings such as multi-tenant clusters and HPC
%clusters with specialized hardware like RDMA.  

\vheading{Redundancy in DNN training}. 
Prior work like Model Batching~\cite{narayanan2018accelerating} %has identified
addressed redundancy in model search %; where an algorithm automatically searches
%or a model architecture for a given task.  However, it
%optimizes for 
when running multiple DNNs together on a single GPU, by
sharing GPU computation across jobs. Our analysis looks at 
the setting where GPUs are not shared between jobs.
OneAccess~\cite{kakaraparthy2019case}  is a preliminary study 
that makes a strong case for %uses reservoir sampling and
%to generate uniformly random samples of data while accessing pre-processed data sequentially.  
%In a departure from the state-of-the-art, 
%OneAccess 
storing pre-processed data across epochs to reduce prep stalls; however such an approach precludes commonly used online data prep techniques %(rescaling, translations, flipping) %and randomization (hue, saturation, brightness, and contrast),
 and this can affect model convergence. %adversely.  %Furthermore, OneAccess uses a simplistic PyTorch baseline with no more than 2 CPU cores used per GPU and very small datasets (MS-COCO~\cite{mscoco} and CIFAR-10~\cite{krizhevsky2009learning}). 
In contrast, \sysname carefully
eliminates redundancy while preserving accuracy and providing significant
speedups.

\begin{comment}
\vheading{Hardware solutions to fetch stalls}. New hardware like NVIDIA's
Magnum IO~\cite{magnum}, and PureStorage's AIRI~\cite{airi}
provide high throughput storage solutions to address  fetch stalls. While these fast hardware may mask 
fetch stalls in some models, they may not help if the model is bottlenecked on prep stalls. 
%\sysname accelerates DNN training by mitigating 
Our work mitigates data stalls  with existing 
commodity servers as opposed to relying on expensive hardware solutions, by efficiently using available hardware.

\end{comment}
\begin{comment}
\vheading{Optimizing DNN training time}.  
 A number of solutions have been proposed to reduce the training time
 for DNNs including specialized hardware~\cite{jouppi2017datacenter,
   jeon2019analysis, tpu, ovtcharov2015accelerating, nurvitadhi2017can,
   putnam2014reconfigurable, cerebras, graphcore}, parallel
 training~\cite{krizhevsky2012imagenet, dean2012deepbelief,
   chilimbi2014adam, jia2018beyond, krizhevsky2014one,
   narayanan2019pipedream, huang2018gpipe}, GPU memory
 optimizations~\cite{vdnn,chen2016training,gist2018}, lowering
 communication overhead~\cite{lin2017dgc, PoseidonATC2017,
   hashemi2018tictac, jayarajan2019priority, nccl, wangt2018blink}, %faster communication
%networking libraries for collective communication
%libraries~\cite{nccl, wangt2018blink}
%, and compiler-based
, and operator optimizations~\cite{vasilache2018tensor, chen2018tvm,
   jia2019taso}. This paper presents a new point in this spectrum, \textit{data stalls}.  


\vheading{Importance of data ingest pipelines}. There is a rich literature in the
database community both in understanding 
data stalls and cache behaviour in DBMS~\cite{vldb99, vldb20_dc, vldb20}, as well 
as building efficient data ingest pipelines for query processing~\cite{pdis96,sigmod98,vldb19}. 
Our work seeks motivation from such findings
and analyses data stalls in the context of emerging DNN workloads.
\end{comment}

\vheading{Domain specific caching}. 
%At the core of \sysname is aDNN-aware caching policy. 
The idea of designing a caching policy that
is aware of application semantics is not new. Stonebraker \etal
highlighted the importance of domain-aware caching for databases~\cite{stonebraker81}. Tomkins \etal show that
informed prefetching and caching  in file systems can  reduce the
execution time of \vio-intensive
applications~\cite{tomkins1997informed}. %Similarly, Liao et.al. show
%that application-aware client side caching in a parallel filesystem
%outperforms traditional caching approaches~\cite{liao2005collective}.
Our work draws parallels to such techniques by first
%identifying data stall times in DNN training,
understanding DNN access pattern and then devising a
caching policy based on these observations.





\begin{comment}
\vheading{Hardware solutions}
New hardware like NVIDIA's Magnum IO~\cite{magnum}, and PureStorage's AIRI~\cite{airi}
provide high throughput storage solutions, and higher CPU cores (4 -- 5 per GPU)
to address data stalls. While these fast hardware may mask stalls in some models, 
it may not help models that need higher number of CPU cores (as shown in analysis).
\sysname accelerates DNN training by mitigating data stalls  
with existing commodity servers as opposed to relying on expensive hardware solutions.
\end{comment}
%Furthermore, as compute gets faster, the bottleneck may shift back to storage. Such high-end hardware solutions are also unavailable in public cloud.


%OneAccess~\cite{kakaraparthy2019case} is a preliminary study on
%storing pre-processed data items on storage to reduce
%prep stalls.  It takes the naive approach of storing pre-processed
%minibatches across epochs, which can adversely affect model convergence. 
%Furthermore, it does not show performance gains over baseline
%PyTorch when more than 2 CPU cores are used per GPU.  
%On the other hand, \sysname carefully
%eliminates redundancy while preserving accuracy and providing significant
%speedups.






\begin{comment}
While both these works aim at reducing fetch stalls
in specific scenarios, unlike \sysname, they neither
accelerate common-case single server training, nor eliminate prep stalls.
Quiver is distributed storage (SSD) cache that
uses a new substitutable sampling technique co-designed
with the PyTorch framework, which restricts
randomness in the creation of minibatches to a subset of cached items. 
Unlike \sysname that accelerates a variety of training 
settings, Quiver is specifically designed for HP search when the dataset 
is too large to fit on the local storage device (> 3TB). DeepIO also proposes an entropy-aware sampling technique, and RDMA based
data shuffling for distributed training across servers.  
However, when the entire dataset does not fit in memory, DeepIO cache suffers from
thrashing unlike \minio. Unlike DeepIO, \sysname does not require any
specialized hardware support.
% and provides impressive speedups over
%commodity TCP stack with low bandwidth requirements and no changes
%to the training framework.
\end{comment}




==> v3/store.tex <==
\section{Mitigating Data Stalls}
\label{sec-design}



Based on the insights from our analysis,
we explore ways of mitigating data stalls using domain specific
techniques that reduces cache misses,
and eliminates redundancy in data fetch and prep.
We further discuss how to reduce the cost of decoding
in ~\sref{sec-disc}.
%\input{existing}

\input{tables/tbl-techniques}



\subsection{The \minio cache}
\label{sec-minio}
As datasets increase in size, they cannot be
cached entirely in the memory of a server during training.
In such cases, DNNs  suffer from fetch stalls if the rate of data fetch 
is lower than the rate of compute (despite prefetching and 
pipelining data fetch with compute) as discussed in (\sref{sec-data-stall}). 
Note that, when fetch stalls occur, training is bottlenecked 
by the bandwidth of storage device, therefore it is crucial to 
minimize \vio by maximizing cache hits every epoch.
% if the
%dataset cannot be fully cached in memory and
%has to be fetched from the storage during training 
%(\sref{sec-data-stall}). Recall from Fig~\ref{fig-rate} 
%that fetch stalls occur when the rate of data fetch 
%is lower than the rate of compute (despite prefetching and 
%pipelining data fetch with compute). 

%There are two ways to reducing
%this fetch stalls; increasing the speed at which uncached
%data items are fetched from storage or increasing the
%amount of cached items. Note that, neither of them are 
%possible without adding additional hardware (faster storage or 
%more DRAM). 

DNN training frameworks today, rely on the OS Page Cache 
to cache the training dataset. However, 
we tap on the piercing insight of Stonebraker \etal's
pioneering work on database caching~\cite{stonebraker81},
 that \emph{the
abstractions provided by OS can hinder the 
development of efficient databases}, and validate
it in the context of DNN 
workloads. Therefore, we study the DNN data access pattern
to design a domain-specific cache \minio.

\input{fig-dali/fig-minio}
%When fetch stalls occur, training proceeds at the rate 
%at which uncached data items can be fetched from storage;
%therefore it is important to minimize the amount of data 
%fetched from storage in each epoch. 
%\minio tackles this problem by ensuring
%that every item in the cache is used effectively in each epoch;
%thereby minimizing the amount of disk IO per epoch to the
%ideal minimum.



%Currently, DNN training platforms rely
%on the OS Page Cache to cache training data. 
%Every data item read from the storage device is cached 
%in the Page Cache to speed up future accesses. 
OS Page Cache works as follows; whenever a 
data item is read from storage, it  is cached 
in the Page Cache to speed up future accesses. 
When the Page Cache reaches its capacity, a 
\emph{cache replacement policy} decides which of the 
existing items to evict to make space for the new one. 
Linux uses a variant of Least Recently Used (LRU)  
for cache replacement~\cite{linux-lru}.

However, DNN training has a unique data access pattern: it is
\textit{repetitive across epochs} and \textit{random within an epoch}.  Training is split into
epochs: each epoch accesses all the data items in the dataset exactly
once in a random order.
We make a key observation about the DNN access pattern that
is at odds with such OS cache replacement policies. \emph{All} data
items in the dataset have equal probability of access in an
epoch. Therefore, it is \emph{not important} which data item is
cached.  Instead, it is crucial that cached items are not replaced
\emph{before} they are used, to minimize storage \vio per epoch.



Therefore, \minio recommends a simple and unintuitive solution;
\emph{items, once cached, are never replaced} in the DNN cache. \minio
works as follows. In the first epoch of the training job, \minio
caches random data items as they are fetched from storage, to populate
the cache. Once the cache capacity is reached, \minio will not evict
any items in the cache; instead, the requests to other data items default to
storage  accesses. The
items in the \minio cache survive across epochs until the end of
the training job. Every epoch beyond the first gets exactly as many hits
as the number of items in the cache; this reduces the per-epoch disk
\vio to the difference in the size of dataset and the cache.

Figure~\ref{fig-minio} contrasts the caching policy of the OS Page Cache
and \minio. Consider a dataset of size 4 (with items A -- D) and a cache of size
2 (50\% cache). Let's say after warmup, the cache has two items D and
B.  Figure~\ref{fig-minio} shows the state of the cache for two
training epochs.  \minio only incurs capacity misses per epoch (here
2); the Page Cache on the other hand, can result in anywhere between
2-4 misses per epoch because of thrashing. For instance, in the first
epoch, D is in the cache to begin with, but kicked out to make way for
a new item C, and later in the same epoch it is requested again (thrashing).  We
empirically verified this using large datasets and varying cache sizes
(\sref{sec-eval}) and found that Page Cache results in close to 20\%
more misses than \minio due to thrashing.


\begin{comment}
\vheading{Prefetching}. While it is possible to add a prefetcher to
the OS Page Cache, we empirically verified that is it detrimental;
prefetcher threads do not play well with each other and evicts
items that were prefetched by other threads in the page cache,
resulting in thrashing. 
While it is possible to add prefetching to \minio by intelligently
replacing items already used in the current epoch by new
prefetched items, we observed that it does not reduce
fetch stalls. Recall that fetch stalls occur when the
rate of compute is faster than storage; when training 
is progressing at the rate of storage throughput, there
is point in prefetching. 
\jm{Someone please help me explain this better if you understand 
what I am getting at $\_/\backslash\_$ }
\end{comment}
%While techniques like prefetching 
%can be added to the \minio cache to increase the effectiveness, it does not reduce total
%disk I/O, and cannot be applied if there is no spare disk bandwidth
%for prefetching. 

\minio's no replacement policy simplifies the design of the
cache as we do not need bookkeeping about the time or frequency
of access of data items. %; if we were to implement a replacement policy, such
%metadata needs to be tracked. 
Moreover, we choose to 
implement \minio in user-space and not as a new replacement policy in the
kernel, making it flexible to use in scenarios where the user has no root privileges to modify the kernel.
The strength of \minio thus lies in its simplicity
and effectiveness.

\vspace{-1em}
\subsection{Partitioned \minio Caching}
\label{sec-part-cache}
\minio reduces the amount of disk \vio (fetch stalls) in single-server training. In
distributed training, the dataset is partitioned and processed by a
group of servers. Each server operates on a random shard of the dataset per epoch,
and this partition changes every epoch (~\sref{sec-etl}).
The \minio cache alone, is not efficient in this setting. For example, consider a
distributed training job across two servers, each of which can
cache 50\% of the dataset. In every epoch, each server has to process
a random 50\% partition of the dataset, some of which may be hits in
the local \minio cache but the misses result in storage \vio, which is
expensive and results in fetch stalls.

We observe that the cross-node network bandwidth in publicly available
cloud GPU instances and our clusters(10-40 Gbps) is upto 4\myx higher than the read
bandwidth of local SATA SSDs (530 MBps).  Data transfer over
commodity TCP stack is much faster than fetching a data item from its
local storage, on a cache miss.  Therefore, we can coordinate the remote \minio
caches across all servers.
%\sysname introduces
%partitioned caching across the DRAM of all servers in the distributed job. 
%While \minio ensures that each
%epoch gets maximum hits in the cache, partitioned cache further reduces
%fetch stalls by increasing the rate at which
%uncached data items are fetched.
% from storage.

Partitioned \minio caching works as follows. In the first epoch, the dataset
is sharded across all servers, and each server populates it's local
\minio cache with data items in the shard assigned to it. At the end
of the first epoch, we collectively cache a part of the dataset
of size equal to the sum of capacities of individual \minio caches.
To route data fetch requests to the appropriate server, we
maintain metadata about data items present in each server's cache.
Whenever a local cache miss happens in the subsequent epoch at any
server, the item is first looked up in the metadata; if present,
it is fetched from the respective server over TCP, else from its local storage.
If the aggregate memory on the participating servers is large enough
to cache the entire dataset, then partitioned caching ensures that
there is no storage \vio on any server beyond the first epoch; the entire
dataset is fetched exactly once from disk in the duration of
distributed training. 
%Partitioned caching scales well as we 
%distribute training across a large number of servers, by caching replicas of the dataset
%if there is more distributed memory than 
%required for the dataset.

% VC: I think we can safely leave out this detail, shouldn't affect
% correctness.
%

% In settings where the local \minio cache has capacity larger than the
% shard assigned to it, \sysname first caches the entire shard and fills
% up any available spots in the background with supplementary items that
% are not in the assigned shard.  Note that while this introduces
% redundancy in the global cache, supplementary items are not added to
% the metadata used by partitioned cache; they are only meant to
% maximize local cache hits. This helps balance the load of data fetch
% requests on each server.

\vspace{-0.5em}
\subsection{Coordinated Prep}
\label{sec-coord-prep}
Hyperparameter (HP) search for a model involves running several
concurrent training jobs, each with a different value for the HP and
picking the best performing one. Our analysis shows that co-locating HP
search jobs on the same server results in both fetch and prep stalls
(\sref{sec-analysis}) due to lack of coordination in data fetch
and prep among these jobs.

We introduce \emph{coordinated prep} to address this
issue. The idea behing coordinated prep is simple. 
Each job in the HP search operates on the same data;
hence, instead of accessing data independently for each job,
they can be coordinated to fetch and prep the dataset exactly once per
epoch. Each epoch is completed in a synchronized fashion by all HP
jobs; as a result, pre-processed minibatches created by one job can be
reused by all concurrent jobs.

Coordinating HP search jobs must be done carefully to ensure that: 
\emph{each job processes the entire dataset exactly
  once per epoch}.  A naive way of doing this is to pre-process the
dataset once and reuse across all HP jobs and all epochs as 
suggested by prior work~\cite{cerebro, kakaraparthy2019case}. This
approach will not work for two reasons. First, reusing pre-processed
data across epochs may result in lower accuracy, as the random
transformations are crucial for learning. Second, the pre-processed items
are 5--7\myx larger in size when compared to the raw data items.
Caching pre-processed items will overflow the system memory capacity
quickly for large datasets. If we store them on storage, we may incur fetch stalls. 

Coordinated prep addresses these challenges by staging pre-processed
minibatches in memory for a short duration \emph{within an
  epoch}. Since each job has identical per-minibatch processing time,
the minibatch is short lived in the staging area.  Coordinated prep
works as follows.

Each HP search job on a server receives a
random shard of the dataset when they start. Each job fetches and
pre-processes the assigned shard, creating minibatches as they
would normally do. When ready, these minibatches 
are exposed to the other jobs in the cross-job staging area. 
This is  a memory region that is 
accessible to all running jobs on the server.
Additionally, each minibatch has a unique ID and an
associated atomic counter that tracks how many
jobs have used this minibatch so far in the current epoch. 
When a job needs a minibatch for GPU processing, it
retrieves it from the staging area and
updates its usage counter. A minibatch is deleted from the 
staging area when it is used exactly once by all running jobs,
as we want to ensure that it is not used across epochs.
We empirically show in \sref{sec-eval} that the
addition of cross-job staging area does not
introduce additional memory overhead.

%Thus, coordinated prep ensures one sweep over the dataset
%per epoch for both data fetch and pre-processing, 
%eliminating redundant work. Note that coordinated
%prep allows addition or removal of jobs only at epoch 
%boundaries; this is not an issue because popular
%HP search algorithms evaluate the
%objective function (for e.g., accuracy),
%and make decisions on terminating or
%continuing the job at epoch boundaries~\cite{jaderberg2017population,
%hyperband}
\begin{comment}
To handle job failures in HP search, we implement a failure detection module to
monitor the status of running jobs. Every prepared minibatch fetched from the staging area 
has an associated timeout. If any job times out waiting for a minibatch,
it notifies the driver process of a possible failure. 
All the jobs can deterministically identify which job failed to 
populate the batch it is waiting on. If the job indeed failed, a new process is spawned 
to resume data loading for the failed shard.
\end{comment}
%The failure detection module verifies if
%the reported job is alive or dead; if
%alive, it issues a broadcast to all the jobs to retry fetching the
%minibatch from staging area, else it spawns a new process to resume
%data loading for the failed shard .
\begin{comment}
\vheading{Handling job failures and terminations}.
The progress of each HP search job in coordinated prep is dependent 
on the progress of all other running jobs, because each job is 
responsible for pre-processing a shard of the dataset. 
Therefore, if one of the jobs is killed by the user in the 
middle of an epoch, or terminates abruptly, all other jobs 
may stall waiting for minibatches that the job was responsible 
for preparing. To address this, 
we use a failure detection module to 
monitor the status of running jobs.

Every prepared minibatch fetched from the staging area 
has an associated timeout.
% We empirically  set this timeout 
% to be equal to the duration of processing 10 minibatches, 
% because it was sufficient to mask the discrepancies in 
% data loading time of individual jobs. 
If any job times out waiting for a minibatch in the staging area,
it notifies the driver process of a possible failure.
% Note that, the global sequence of data items 
% seen by each job is identical; therefore,
All the jobs can deterministically identify which job failed to 
populate the batch it is waiting on. The failure detection module verifies if
the reported job is alive or dead; if
alive, it issues a broadcast to all the jobs to retry fetching the
minibatch from staging area, else it spawns a new process to resume
data loading for the failed shard .
\end{comment}

\subsection{Tying it all together with \sysname}
We implement the three techniques discussed thus far as a part of 
a user-space data loading library, \sysname. We build \sysname
on top of DALI to take advantage of the GPU-accelerated data 
pre-processing operations. %Unlike existing systems like
%Quiver or Cerebro, 
\sysname can be used as a drop-in replacement
for the default PyTorch dataloader. %, with no changes to the cluster infra. 



The overall architecture of \sysname is as follows. %shown in 
%Figure~\ref{fig-recall}. 
The training dataset resides on a local
storage device like SSD/HDD. If the data resides on a remote
storage service, it is cached in local storage when first
accessed~\cite{blobfuse}. For all later epochs, the data is
fetched from local storage. In each training iteration, a minibatch of
data must be fetched from disk (or cache), pre-processed to apply
random transformations and collated to a tensor that can be copied
over to the GPU for computation. \sysname manages its
own \minio cache of the raw data items (before any stochastic
pre-processing transformations are applied).  The data sampling and
randomization is unmodified; in each epoch, every minibatch is
sampled randomly from the dataset. Every data item is then subjected
to the random pre-processing pipeline specified in the training
workload. The prepared minibatch is then placed in a cross-job staging
area for consumption by the GPU. If a single data-parallel job is
running across multiple GPUs in a server, then the minibatches in the
staging are used exactly once per epoch and discarded; if there are
concurrent HP jobs on a server, then the staging area retains
minibatches until each concurrent job has used it exactly once in the
current epoch. Any minibatch that satisfies this criteria is evicted
from the staging area to make way for newer batches.




==> v3/tool.tex <==
\section{\tool : Predictive analysis}
While all the experiments \revision{that vary cache size, and the number of
CPU cores} in \sref{sec-data-stall} are run on physical
servers, we extend \tool to help a user simulate these experiments
without having to run all different configurations on physical
servers.  
\revision{While there exists prior work that predict the performance of
a DNN, they focus on profiling the layer-wise
performance of DNN~\cite{tpu-tools, mxnet-profile},
low level perf counters for accelerators~\cite{nvidia-profile, iyer2016gpu},
or finding optimization opportunities at the neural network 
layer level~\cite{zhu2020daydream}. 
In contrast, \tool analyzes the
implication of CPU, memory, and storage
on the performance of a DNN and answers what-if questions.}
% such
%as, how much DRAM does the model need to avoid 
%fetch stalls, how many CPU cores should each GPU use
%for pre-processing to eliminate prep stalls, and so on.

%\tool profiles the given model once on the server;
%using the metrics collected, it can answer what-if questions such as,
%how much cache does the model need to mask fetch stalls, how many
%CPU cores should each GPU use  to eliminate prep
%stalls, and so on.  
This is a powerful means of analyzing whether
throwing more hardware at the problem will solve the issue of data
stalls. For instance, if training is dominated by fetch stalls
(bottlenecked on disk bandwidth), then increasing the number of CPU
cores on the machine has no benefit; either DRAM capacity has to be
increased, or the disk must be replaced with a higher bandwidth
one. Similarly, if the training job is bottlenecked on prep,
then increasing DRAM has no effect on training time.  \revision{\tool is useful
in scenarios like this, to predict the performance of a model as we
scale up CPU, memory, or storage. However, \tool needs to be run 
atleast once for every new GPU and DNN architecture to collect the required information,
and predicts the impact of varying auxiliary resources like CPU, memory, or storage on data stalls.}


%\input{fig-analysis/fig-rates}
\vheading{Estimating data stalls}.
%Figure~\ref{fig-rate} shows the 
Consider the different components involved in a typical DNN  
data pipeline as in Figure~\ref{fig-rate}; 
data is fetched from cache (and store) with an effective 
prefetch rate $F$, pre-processed at the CPU at a rate $P$ and
processed at the GPU at a rate $G$. 
To perform predictive analysis, \tool measures 
several metrics related to the data pipeline of the model;
the maximum ingestion rate at the GPU $(G)$, the rate 
of CPU prep $(P)$, the
rate of cache fetch $(C)$, and the rate of storage fetch $(S)$,
by training for a fixed number of iterations (default:100) using the
differential technique discussed in \sref{sec-tool}. More details on
how \tool measures these quantities is precisely mentioned in our 
Technical Report~\cite{coordl-arxiv}.
%These quantities are measured in samples per second. 
Using these metrics,
\tool models the training iteration %can estimate the effective prefetch rate $(F)$, and
to answer what-if questions such as, how much
DRAM cache is required for this model to
eliminate fetch stalls? %What happens if
%the GPU compute is 2\myx faster?, etc. 
\begin{comment}
\tool 
collects these metrics for a model as follows.

\vheading{(i) Measure ingestion rate $(G)$}. To find the
maximum possible speed at which the DNN can train, 
\tool first runs the job script for a fixed number iterations (default:100)
with synthetic data that is pre-populated at the GPUs.
It then calculates $G$ as,
\vspace{-0.5em}
\begin{equation}
G = \frac{\mbox{Total samples processed in (i)}}{\mbox{Time for (i)}} \\
\vspace{-1.5em}
\label{eq-gpu}
\end{equation}

\begin{equation}
\mbox{Samples processed} = \mbox{\#iterations} \times \mbox{global batch size}\\
\end{equation}

\vheading{(ii) Measure prep rate $(P)$}. Next, \tool
executes the training script with the given dataset
by ensuring that the subset of data used is cached in 
memory, using all available CPU cores. Additionally,
the GPU computation is disabled to only run the 
data loader. This is required because, if $P \geq G$,
then we cannot measure P using the knowledge of
runs (i) and (ii), as prep will be pipelined
with GPU compute. Therefore, \tool disables
GPU computation and estimates P in the same way
as Eq~\eqref{eq-gpu}.


\vheading{(iii) Measure storage fetch rate $(S)$}.
Storage fetch rate is the maximum random
read throughput of the storage device. To measure
this, \tool runs the data loader (with a cold cache,
disabling both pre-processing and GPU compute), with
all CPU cores.

\vheading{(iv) Measure cache fetch rate $(C)$}.
To measure the rate at which data can be fetched 
from cache, \tool uses a microbenchmark to 
measure memory bandwidth and uses it as an 
approximation for $C$. Note that run (ii) actually
includes the time to fetch cached items as well;
however we see that the cache fetch rate is very high 
(few tens of GBps), and does not add noise to the
measurement of prep rate.

\end{comment}

%A comprehensive list of data pipeline rates ($G, P, F$) for several models, datasets, 
%and configurations in the Appendix of our TR~\cite{coordl-arxiv}.

%\input{tables/tbl-tool}
\input{fig-analysis/fig-tool}
\subsection{Example : Predicting optimal cache size}
We now describe an example of what-if analysis with
\tool. We show how \tool answers the question : 
\emph{how much DRAM cache does the DNN need to eliminate 
	fetch stalls?}
To predict the implication of cache size, \tool 
calculates the effective prefectch rate $(F)$ for 
a given cache size $(x$ \% of the dataset). Here, we assume that
the cache implements an efficient policy like
\minio; i.e., a cache of size $x$ items has atleast
$x$ hits per epoch. $F$ is computed as follows. Say the size of the dataset is
$D$ samples, and cache is $x\%$ of the dataset. Therefore,
in an epoch, the total time to read the dataset is given by
\vspace{-0.6em}
\begin{equation}
T_f = \frac{D \times x}{C} + \frac{D \times (1-x)}{S} \\
\label{eq-fetch-time}
\end{equation}

The fetch rate is then calculated as,
\begin{equation}
F = \frac{D}{T_f} = \frac{D}{\frac{D \times x}{C} + \frac{D \times (1-x)}{S}}\\
\label{eq-fetch}
\end{equation}

Since $C >> S$, $F \propto \frac{1}{1-x}$, i.e, the effective fetch
rate increases, as the number of uncached items per epoch decreases.
Since \tool has already estimated values of $D$, $C$, and $S$, given a 
cache percentage $x$, \tool can predict the fetch rate using Eq~\eqref{eq-fetch}.

\begin{comment}
Then, using $F$, $P$, and $G$, it is easy to see where the 
bottleneck in training is; 

If $min(F,P,G) = G$, then the training is GPU-bound

If $min(F,P,G) = P$, then the training is CPU-bound

If $min(F,P,G) = F$, then the training is IO-bound \\
\end{comment}


To evaluate how accurately \tool can 
answer this question, we run the actual experiment by
varying cache size on a physical server (empirical), and %$(F_{empirical})$, and
comparing it to the predictions of \tool %$(F_{predicted})$
for AlexNet on \confssd with Imagenet-1K.  %Predicted training speed is $min(F,P,G)$.
 Figure~\ref{fig-tool-cache} plots the predicted 
values of $F$, $P$, and $G$, alongside empirical speed while
varying cache size. First, we observe that  the predicted training speed
($min(F,P,G)$) is a maximum of
4\% off the empirical results. Second, using these predictions, \tool
can estimate the optimal cache size for the model 
by comparing it with prep rate (P) and GPU ingestion rate (G). 
To eliminate fetch stalls, $F > min(P,G)$ as shown by the intersection 
in Figure~\ref{fig-tool-cache}.  At lower cache sizes,
training is \vio bound, however, a cache that is 
50\% of the dataset size is sufficient to eliminate fetch stalls;
larger cache (more DRAM) is not beneficial beyond this point,
as training becomes CPU-bound. %Figure~\ref{fig-tool-cache}
%shows that empirical training speed observed from experiments 
%with varying cache sizes on real hardware
%shows the same trend predicted by \tool.
A comprehensive list of data pipeline rates ($G, P, F$) for several models, datasets, 
and configurations in the Appendix of our Technical Report~\cite{coordl-arxiv}.

%Note that the prep rate is much lower 
%than the GPU ingestion rate; to eliminate this prep stall,
%we either need to add more CPU cores, or use techniques like
%coordinated prep to inch closer to the GPU ingestion rate.

